Recent developments and research needs in turbulence modeling of hypersonic flows

Hypersonic flow conditions pose exceptional challenges for Reynolds-Averaged Navier-Stokes (RANS) turbulence modeling. Critical phenomena include compressibility effects, shock/turbulent boundary layer interactions, turbulence-chemistry interaction in thermo-chemical non-equilibrium, and ablation-induced surface roughness and blowing effects. This comprehensive review synthesizes recent developments in adapting turbulence models to hypersonic applications, examining approaches ranging from empirical modifications to physics-based reformulations and novel data-driven methodologies. We provide a systematic evaluation of current RANS-based turbulence modeling capabilities, comparing eddy viscosity and Reynolds stress transport formulations in their ability to predict engineering quantities of interest such as separation characteristics and wall heat transfer. Our analysis encompasses the latest experimental and direct numerical simulation datasets for validation, specifically addressing two- and three-dimensional equilibrium turbulent boundary layers and shock/turbulent boundary layer interactions across both smooth and rough surfaces. Key multi-physics considerations including catalysis and ablation phenomena along with the integration of conjugate heat transfer into a RANS solver for efficient design of a thermal protection system are also discussed. We conclude by identifying the critical gaps in the available validation databases and limitations of the existing turbulence models and suggest potential areas for future research to improve the fidelity of turbulence modeling in the hypersonic regime.

==> EXTRA-REFS-FROM-JFM-FORMAT <==
@article{daly1970transport,
  title={Transport equations in turbulence},
  author={Daly, Bart J and Harlow, Francis H},
  journal={Physics of fluids},
  volume={13},
  number={11},
  pages={2634--2649},
  year={1970}
}

@article{zhao2020rans,
  title={RANS turbulence model development using CFD-driven machine learning},
  author={Zhao, Yaomin and Akolekar, Harshal D and Weatheritt, Jack and Michelassi, Vittorio and Sandberg, Richard D},
  journal={Journal of Computational Physics},
  volume={411},
  pages={109413},
  year={2020},
  publisher={Elsevier}
}

@article{singh2017machine,
  title={Machine-learning-augmented predictive modeling of turbulent separated flows over airfoils},
  author={Singh, Anand Pratap and Medida, Shivaji and Duraisamy, Karthik},
  journal={AIAA journal},
  volume={55},
  number={7},
  pages={2215--2227},
  year={2017},
  publisher={American Institute of Aeronautics and Astronautics}
}

@article{parish2016paradigm,
  title={A paradigm for data-driven predictive modeling using field inversion and machine learning},
  author={Parish, Eric J and Duraisamy, Karthik},
  journal={Journal of computational physics},
  volume={305},
  pages={758--774},
  year={2016},
  publisher={Elsevier}
}

@article{duraisamy2021perspectives,
  title={Perspectives on machine learning-augmented Reynolds-averaged and large eddy simulation models of turbulence},
  author={Duraisamy, Karthik},
  journal={Physical Review Fluids},
  volume={6},
  number={5},
  pages={050504},
  year={2021},
  publisher={APS}
}

@article{abe2001towards,
  title={Towards the development of a Reynolds-averaged algebraic turbulent scalar-flux model},
  author={Abe, K and Suga, K},
  journal={International Journal of Heat and Fluid Flow},
  volume={22},
  number={1},
  pages={19--29},
  year={2001},
  publisher={Elsevier}
}

@article{shin2008elliptic,
  title={Elliptic relaxation second moment closure for the turbulent heat fluxes},
  author={Shin, Jong Keun and An, Jeong Soo and Choi, Young Don and Kim, Young Chan and Kim, Min Soo},
  journal={Journal of Turbulence},
  number={9},
  pages={N3},
  year={2008},
  publisher={Taylor \& Francis}
}

@article{weatheritt2020data,
  title={Data-driven scalar-flux model development with application to jet in cross flow},
  author={Weatheritt, Jack and Zhao, Yaomin and Sandberg, Richard D and Mizukami, Satoshi and Tanimoto, Koichi},
  journal={International Journal of Heat and Mass Transfer},
  volume={147},
  pages={118931},
  year={2020},
  publisher={Elsevier}
}

@article{lozano2023machine,
  title={Machine learning building-block-flow wall model for large-eddy simulation},
  author={Lozano-Dur{\'a}n, Adri{\'a}n and Bae, H Jane},
  journal={Journal of Fluid Mechanics},
  volume={963},
  pages={A35},
  year={2023},
  publisher={Cambridge University Press}
}

@techreport{boseuse,
  title={The Use of Probabilistic Modeling for Reentry Thermal Protection System Design},
  author={Bose, Deepak and Wright, Michael J and Mansour, Nagi N},
  institution={Tech. rep., RTO-MP-AVT-147}
}


@article{longo2004modelling,
  title={Modelling of hypersonic flow phenomena},
  author={Longo, JMA},
  journal={Critical Technologies for Hypersonic Vehicle Development Technology--RTO/AVT/VKI Lecture Series},
  pages={10--14},
  year={2004},
  publisher={Citeseer}
}
@article{Hoste2024,
  title={A review of {RANS} modeling for hypersonic large cone-flares},
  author={Hoste, J.-J. and Gibbons, N. and Ecker, T. and Amato, C. and Knight, D. and Sattarov, A and Thiry, O. and Hickey, J.-P. and Hizir, F.E.  and K\"{o}kt\"{u}rk, T. and Castelino, N. and Viti, V. and Roldan, M. and Qiang, S. and Coder, J. and Baurle, R. and White, J. },
  journal={Physics of Fluids},
  volume={(under review)},
  number={},
  pages={},
  year={2024}
}

@article{CHRISTOPHER2020,
title = {DNS of turbulent flat-plate flow with transpiration cooling},
journal = {International Journal of Heat and Mass Transfer},
volume = {157},
pages = {119972},
year = {2020},
issn = {0017-9310},
doi = {https://doi.org/10.1016/j.ijheatmasstransfer.2020.119972},
url = {https://www.sciencedirect.com/science/article/pii/S0017931019355656},
author = {Nicholas Christopher and Johannes M.F. Peter and Markus J. Kloker and Jean-Pierre Hickey},
keywords = {Transpiration cooling, Compressible DNS, Turbulent boundary layer, Cooling efficiency},
abstract = {Transpiration cooling in a turbulent boundary layer on a flat plate is investigated using direct numerical simulations (DNS). The simulations are performed by solving the compressible Navier-Stokes equations at low Mach number conditions (M∞=0.3). Both the coolant and the hot gas are air, with isothermal walls and coolant at a temperature of Tw/T∞=0.5, while the blowing ratio and boundary conditions have been varied. These simulations elucidate the turbulence and heat-flux alterations due to the interaction of the coolant with the hot-gas boundary layer. By increasing the blowing ratio, the peak turbulent kinetic energy moves away from the wall to a region of shear between the low-momentum coolant and high-momentum hot gas. The reduction of the wall heat transfer is caused by the combined effects of heat advection due to the non-zero wall-normal velocity at the wall, and the reduction of the average boundary-layer temperature due to the accumulation of coolant. A new model for the latter effect is proposed which is physically realistic in the limit cases. The proposed combined model accounts for both heat advection and film accumulation and shows good agreement with the DNS data. An increase in turbulent transport of heat with increasing blowing rate is caused by the production of vortices between the coolant and hot gas. This causes a reduction in the cooling effectiveness, and can be seen near the leading edge of the transpiration region. In order to investigate wall modelling effects, simulations with uniform coolant injection have been compared to simulations with injection via many small strips. It is observed that as the strips get smaller (at fixed total mass flow rate and fixed wall porosity), the results trend towards the uniform injection case. Therefore, it is hypothesized that for small pore sizes, neglecting the effects of the individual pores in the wall boundary condition is physically justifiable.}
}

@article{Bukva2021,
    author = {Bukva, Alexander and Zhang, Kevin and Christopher, Nicholas and Hickey, Jean-Pierre},
    title = {Assessment of turbulence modeling for massively-cooled turbulent boundary layer flows with transpiration cooling},
    journal = {Physics of Fluids},
    volume = {33},
    number = {9},
    pages = {095114},
    year = {2021},
    month = {09},
    abstract = {We assess Reynolds-averaged Navier–Stokes (RANS) turbulent closures for the prediction of a turbulent boundary layer with transpiration cooling via comparison with a high-fidelity direct numerical simulation database. This study considers the canonical zero-pressure gradient, flat-plate, turbulent boundary layer over a massively cooled wall, with transpiration cooling. The simulations are conducted at a low-subsonic Mach number and we study two transpiration cooling configurations with uniform and slit injection at various blowing ratios. The DNS and RANS simulation setups are nearly identical. The RANS-based turbulence models perform well in the qualitative estimation of the velocity and thermal boundary layer evolution at low-blowing ratios (F = 0.2 and 0.6\%); more significant differences are noted at higher blowing ratios (F=2.0\%). The RANS models, especially the Spalart–Allmaras model, over-predict turbulence production near the wall which results in faster growth in the boundary thickness; this error becomes more pronounced at higher blowing ratios. Despite the greater mixing of momentum, the thermal mixing is under-predicted compared to the DNS in the uniform blowing case but over-predicted for the slit case. These results suggest that modeling errors in the temperature distribution due to turbulent thermal flux modeling can be significant even if the velocity is correctly modeled.},
    issn = {1070-6631},
    doi = {10.1063/5.0062155},
    url = {https://doi.org/10.1063/5.0062155},
    eprint = {https://pubs.aip.org/aip/pof/article-pdf/doi/10.1063/5.0062155/13883731/095114\_1\_online.pdf},
}


@InProceedings{holden2013measurements,
  author    = {Holden, MS and Wadhams, TP and MacLean, MG},
  booktitle = {21st AIAA Computational Fluid Dynamics Conference},
  title     = {Measurements in Regions of Shock Wave/Turbulent Boundary Layer Interaction from Mach 4 to 10 for Open and “Blind” Code Evaluation/Validation},
  year      = {2013},
  pages     = {2836},
}


@article{mansour2024flow,
  title={Flow Mechanics in Ablative Thermal Protection Systems},
  author={Mansour, Nagi N and Panerai, Francesco and Lachaud, Jean and Magin, Thierry},
  journal={Annual Review of Fluid Mechanics},
  volume={56},
  number={1},
  pages={549--575},
  year={2024},
  publisher={Annual Reviews}
}
@article{schneider2010hypersonic,
  title={Hypersonic boundary-layer transition with ablation and blowing},
  author={Schneider, Steven P},
  journal={Journal of Spacecraft and Rockets},
  volume={47},
  number={2},
  pages={225--237},
  year={2010}
}


@article{park1989nonequilibrium,
  title={Nonequilibrium hypersonic aerothermodynamics},
  author={Park, Chul},
  year={1989}
}

@article{direnzo2021direct,
  title={Direct numerical simulation of a hypersonic transitional boundary layer at suborbital enthalpies},
  author={Di Renzo, M. and Urzay, J.},
  journal={Journal of Fluid Mechanics},
  volume={912},
  year={2021},
  publisher={Cambridge University Press}
}
@article{di2024stagnation,
  title={Stagnation enthalpy effects on hypersonic turbulent compression corner flow at moderate Reynolds numbers},
  author={Di Renzo, M and Williams, CT and Pirozzoli, S},
  journal={Physical Review Fluids},
  volume={9},
  number={3},
  pages={033401},
  year={2024},
  publisher={APS}
}
@article{volpiani2021numerical,
  title={Numerical strategy to perform direct numerical simulations of hypersonic shock/boundary-layer interaction in chemical nonequilibrium},
  author={Volpiani, Pedro Stefanin},
  journal={Shock Waves},
  volume={31},
  number={4},
  pages={361--378},
  year={2021},
  publisher={Springer}
}


@article{colonna2001numerical,
  title={Numerical methods to solve Euler equations in one-dimensional steady nozzle flow},
  author={Colonna, G and Tuttafesta, M and Giordano, D},
  journal={Computer physics communications},
  volume={138},
  number={3},
  pages={213--221},
  year={2001},
  publisher={Elsevier}
}

@article{park2001chemical,
  title={Chemical-kinetic parameters of hyperbolic earth entry},
  author={Park, Chul and Jaffe, Richard L and Partridge, Harry},
  journal={Journal of Thermophysics and Heat transfer},
  volume={15},
  number={1},
  pages={76--90},
  year={2001}
}

@inproceedings{park1988two,
  title="{Two-temperature interpretation of dissociation rate data for N2 and O2}",
  author="Park, C.",
  booktitle="26th Aerspace Sciences Meeting",
  pages="458",
  year="1988"
}


@Article{	  pecnik2017scaling,
  title		= {Scaling and modelling of turbulence in variable property
		  channel flows},
  author	= {Pecnik, R. and Patel, A.},
  journal	= {Journal of Fluid Mechanics},
  year		= {2017},
  pages		= {R1-1--11},
  volume	= {823}
}

@Article{   otero2018turbulence,
  title   = {Turbulence modelling for flows with strong variations in thermo-physical
properties},
  author  = {Otero, G. and Patel, A. and Diez, R. and Pecnik, R.},
  journal = {Journal of Heat and Fluid Flow},
  year    = {2018},
  pages   = {R1},
  volume  = {823}
}

@article{hasan2023incorporating,
  title={Incorporating intrinsic compressibility effects in velocity transformations for wall-bounded turbulent flows},
  author={Hasan, Asif Manzoor and Larsson, Johan and Pirozzoli, Sergio and Pecnik, Rene},
  journal={Physical Review Fluids},
  volume={8},
  number={11},
  pages={L112601},
  year={2023},
  publisher={APS}
}


@article{bowersox2009extension,
  title={Extension of equilibrium turbulent heat flux models to high-speed shear flows},
  author={Bowersox, Rodney DW},
  journal={Journal of fluid mechanics},
  volume={633},
  pages={61--70},
  year={2009},
  publisher={Cambridge University Press}
}
@article{bowersox2010algebraic,
  title={Algebraic turbulent energy flux models for hypersonic shear flows},
  author={Bowersox, Rodney DW and North, Simon W},
  journal={Progress in Aerospace Sciences},
  volume={46},
  number={2-3},
  pages={49--61},
  year={2010},
  publisher={Elsevier}
}

@article{spalding1971concentration,
  title={Concentration fluctuations in a round turbulent free jet},
  author={Spalding, DB},
  journal={Chemical Engineering Science},
  volume={26},
  number={1},
  pages={95--107},
  year={1971},
  publisher={Elsevier}
}

@article{launder2005heat,
  title={Heat and mass transport},
  author={Launder, Brian E},
  journal={Turbulence},
  pages={231--287},
  year={2005},
  publisher={Springer}
}

@article{marquardt2020experimental,
  title={Experimental investigation of the turbulent Schmidt number in supersonic film cooling with shock interaction},
  author={Marquardt, Pascal and Klaas, Michael and Schr{\"o}der, Wolfgang},
  journal={Experiments in Fluids},
  volume={61},
  number={7},
  pages={160},
  year={2020},
  publisher={Springer}
}

@article{tominaga2007turbulent,
  title={Turbulent Schmidt numbers for CFD analysis with various types of flowfield},
  author={Tominaga, Yoshihide and Stathopoulos, Ted},
  journal={Atmospheric Environment},
  volume={41},
  number={37},
  pages={8091--8099},
  year={2007},
  publisher={Elsevier}
}

@article{xiang2020turbulence,
  author =        {Xiang, Z. and Yang, S. and Xie, S. and Li, J. and
                   Ren, H.},
  journal =       {Engineering Applications of Computational Fluid
                   Mechanics},
  number =        {1},
  pages =         {1546--1561},
  publisher =     {Taylor \& Francis},
  title =         {Turbulence--chemistry interaction models with
                   finite-rate chemistry and compressibility correction
                   for simulation of supersonic turbulent combustion},
  volume =        {14},
  year =          {2020},
  doi = {10.1080/19942060.2020.1842248},
}

@article{bray2006finite,
  author =        {Bray, K. N. C. and Champion, M. and Libby, P. A. and
                   Swaminathan, N.},
  journal =       {Combustion and Flame},
  number =        {4},
  pages =         {665--673},
  publisher =     {Elsevier},
  title =         {Finite rate chemistry and presumed PDF models for
                   premixed turbulent combustion},
  volume =        {146},
  year =          {2006},
  doi = {10.1016/j.combustflame.2006.07.001},
}

@inbook{baranwal2020vibrational,
  author =        {Baranwal, A. and Donzis, D. A. and Bowersox, R. D.},
  booktitle =     {AIAA Scitech 2020 Forum},
  pages =         {2052},
  title =         {Vibrational turbulent Prandtl number in flows with
                   thermal non-equilibrium},
  year =          {2020},
  doi = {10.2514/6.2020-2052},
}

@conference{BaPaJo24,
        author = {Matthew Barone and Eric Parish and Cyrus Jordan}, 
        booktitle = {AIAA SciTech},
        date-added = {2023-12-04 10:40:13 -0600},
        date-modified = {2023-12-04 10:41:01 -0600},
        title = {{Data-Driven Modifications to the Spalart--Allmaras Turbulence
Model for Supersonic and Hypersonic Boundary Layers}},
        year = {2024}}

@conference{PaChMi23,
        abstract = { View Video Presentation: https://doi.org/10.2514/6.2023-2126.vidThe Reynolds-averaged Navier--Stokes (RANS) equations remain a workhorse technology for simulating compressible fluid flows of practical interest. Due to model-form errors, however, RANS models can yield erroneous predictions that preclude their use on mission-critical problems. This work presents a data-driven turbulence modeling strategy aimed at improving RANS models for compressible fluid flows. The strategy outlined has three core aspects: (1) prediction for the discrepancy in the Reynolds stress tensor and turbulent heat flux via machine learning (ML), (2) estimating uncertainties in ML model outputs via out-of-distribution detection, and (3) multi-step training strategies to improve feature-response consistency. Results are presented across a range of cases publicly available on NASA's turbulence modeling resource involving wall-bounded flows, jet flows, and hypersonic boundary layer flows with cold walls. We find that one ML turbulence model is able to provide consistent improvements for numerous quantities-of-interest across all cases. },
        author = {Eric Parish and David S. Ching and Nathan E. Miller and Steven J. Beresh and Matthew F. Barone},
        booktitle = {AIAA SCITECH 2023 Forum},
        year = {2023},
        doi = {10.2514/6.2023-2126},
        eprint = {https://arc.aiaa.org/doi/pdf/10.2514/6.2023-2126},
        title = {{Turbulence modeling for compressible flows using discrepancy
tensor-basis neural networks and extrapolation detection}},
        url = {https://arc.aiaa.org/doi/abs/10.2514/6.2023-2126},
        bdsk-url-1 = {https://arc.aiaa.org/doi/abs/10.2514/6.2023-2126},
        bdsk-url-2 = {https://doi.org/10.2514/6.2023-2126}}
}

@phdthesis{Ni24,
        author = {Gary Nicholson}, 
        school = {Ohio State University},
        title = {{Simulation and Modeling of Hypersonic Turbulent Boundary
Layers Subject to Favorable and Adverse Pressure Gradients
Due to Streamline Curvature }},
        year = {2024}}
        

@phdthesis{Jo23,
        author = {Cyrus Jordan}, 
        date-added = {2024-06-07 16:46:01 -0500},
        date-modified = {2024-06-07 16:46:40 -0500},
        school = {North Carolina State University},
        title = {{Turbulence Model Development for Hypersonic Shock Wave
Boundary Layer Interactions }},
        year = {2023}}
        
@article{WaHuDuXi19,
        abstract = {Modeled Reynolds stress is a major source of model-form uncertainties in Reynolds-averaged Navier--Stokes (RANS) simulations. Recently, a physics-informed machine learning (PIML) approach has been proposed for reconstructing the discrepancies in RANS-modeled Reynolds stresses. The merits of the PIML framework have been demonstrated in several canonical incompressible flows. However, its performance on high-Mach-number flows is still not clear. In this work, we use the PIML approach to predict the discrepancies in RANS-modeled Reynolds stresses in high-Mach-number flat-plate turbulent boundary layers by using an existing DNS database. Specifically, the discrepancy function is first constructed using a DNS training flow and then used to correct RANS-predicted Reynolds stresses under flow conditions different from the DNS. The machine learning technique is shown to significantly improve RANS-modeled turbulent normal stresses, the turbulent kinetic energy, and the Reynolds stress anisotropy. Improvements are consistently observed when different training datasets are used. Moreover, a high-dimensional visualization technique and a distance metrics are used to provide a priori assessment of prediction confidence based only on RANS simulations. This study demonstrates that the PIML approach is a computationally affordable technique for improving the accuracy of RANS-modeled Reynolds stresses for high-Mach-number turbulent flows when there is a lack of experiments and high-fidelity simulations.},
        author = {Wang, Jian-Xun and Huang, Junji and Duan, Lian and Xiao, Heng},
        date = {2019/02/01},
        date-added = {2023-05-16 07:40:48 -0500},
        date-modified = {2023-05-16 07:40:48 -0500},
        doi = {10.1007/s00162-018-0480-2},
        id = {Wang2019},
        isbn = {1432-2250},
        journal = {Theoretical and Computational Fluid Dynamics},
        number = {1},
        pages = {1--19},
        title = {{Prediction of Reynolds stresses in high-Mach-number turbulent
boundary layers using physics-informed machine learning}},
        url = {https://doi.org/10.1007/s00162-018-0480-2},
        volume = {33},
        year = {2019},
        bdsk-url-1 = {https://doi.org/10.1007/s00162-018-0480-2}}


@article{passiatore2022thermochemical,
  title={Thermochemical non-equilibrium effects in turbulent hypersonic boundary layers},
  author={Passiatore, Donatella and Sciacovelli, Luca and Cinnella, Paola and Pascazio, G},
  journal={Journal of Fluid Mechanics},
  volume={941},
  pages={A21},
  year={2022},
  publisher={Cambridge University Press}
}

@article{passiatore2023shock,
  title={Shock impingement on a transitional hypersonic high-enthalpy boundary layer},
  author={Passiatore, Donatella and Sciacovelli, Luca and Cinnella, Paola and Pascazio, Giuseppe},
  journal={Physical Review Fluids},
  volume={8},
  number={4},
  pages={044601},
  year={2023},
  publisher={APS}
}


@book{gnoffo1989conservation,
  title={Conservation equations and physical models for hypersonic air flows in thermal and chemical nonequilibrium},
  author={Gnoffo, Peter A},
  volume={2867},
  year={1989},
  publisher={National Aeronautics and Space Administration, Office of Management~…}
}

@article{roy2006review,
  title={Review and assessment of turbulence models for hypersonic flows},
  author={Roy, Christopher J and Blottner, Frederick G},
  journal={Progress in aerospace sciences},
  volume={42},
  number={7-8},
  pages={469--530},
  year={2006},
  publisher={Elsevier}
}


@inproceedings{smits2009current,
  title={Current status of basic research in hypersonic turbulence},
  author={Smits, Lex and Martin, Pino and Girimaji, Sharath},
  booktitle={47th AIAA Aerospace Sciences Meeting including The New Horizons Forum and Aerospace Exposition},
  pages={151},
  year={2009}
}

@inproceedings{brown2002turbulence,
  title={Turbulence model validation for hypersonic flows},
  author={Brown, James},
  booktitle={8th AIAA/ASME Joint Thermophysics and Heat Transfer Conference},
  pages={3308},
  year={2002}
}

@techreport{marvin1989turbulence,
  title={Turbulence modeling for hypersonic flows},
  author={Marvin, Joseph G and Coakley, Thomas J},
  year={1989}
}

@article{marvin1992turbulence,
  title={Turbulence modeling for hypersonic flows},
  author={Marvin, JG and Coakley, TJ},
  journal={Advances in Hypersonics: Modeling Hypersonic Flows},
  pages={1--43},
  year={1992},
  publisher={Springer}
}

@article{degrez1993shock,
  title={Shock-wave/boundary-layer interaction in supersonic and hypersonic flows},
  author={Degrez, G and Simeonides, G and Delery, J and Vandromme, D and Dolling, D and Knight, D and Settles, G},
  journal={AGARD Report},
  volume={792},
  year={1993}
}

@article{bose2013uncertainty,
  title={Uncertainty assessment of hypersonic aerothermodynamics prediction capability},
  author={Bose, Deepak and Brown, James L and Prabhu, Dinesh K and Gnoffo, Peter and Johnston, Christopher O and Hollis, Brian},
  journal={Journal of Spacecraft and Rockets},
  volume={50},
  number={1},
  pages={12--18},
  year={2013}
}

@article{georgiadis2014status,
  title={Status of turbulence modeling for hypersonic propulsion flowpaths},
  author={Georgiadis, Nicholas J and Yoder, Dennis A and Vyas, Manan A and Engblom, William A},
  journal={Theoretical and Computational Fluid Dynamics},
  volume={28},
  pages={295--318},
  year={2014},
  publisher={Springer}
}

@inproceedings{goldberg2005hypersonic,
  title={Hypersonic turbulent flow predictions using CFD++},
  author={Goldberg, Uriel},
  booktitle={AIAA/CIRA 13th International Space Planes and Hypersonics Systems and Technologies Conference},
  pages={3214},
  year={2005}
}

@inproceedings{huang1993turbulence,
  title={Turbulence modeling for complex hypersonic flows},
  author={Huang, P and Coakley, T},
  booktitle={31st Aerospace Sciences Meeting},
  pages={200},
  year={1993}
}

@inproceedings{maicke2010evaluation,
  title={Evaluation of CFD codes for hypersonic flow modeling},
  author={Maicke, Brian and Barber, Timothy and Majdalani, Joe},
  booktitle={46th AIAA/ASME/SAE/ASEE joint propulsion conference \& exhibit},
  pages={7184},
  year={2010}
}

@inproceedings{marvin1992cfd,
  title={A CFD validation roadmap for hypersonic flows},
  author={Marvin, Joseph G},
  booktitle={Fluid Dynamics Panel Meeting and Symposium on Theoretical and Experimental Methods in Hypersonic Flows},
  number={NASA-TM-103935},
  year={1992}
}

@techreport{coakley1994turbulence,
  title={Turbulence compressibility corrections},
  author={Coakley, TJ and Horstman, CC and Marvin, JG and Viegas, JR and Bardina, JE and Huang, PG and Kussoy, MI},
  year={1994}
}

@inproceedings{paciorri1997validation,
  title={Validation of the Spalart-Allmaras turbulence model for application in hypersonic flows},
  author={Paciorri, Renato and Dieudonne, W and Degrez, G and Charbonnier, J-M and Deconinck, H and Paciorri, R and Dieudonne, W and Degrez, G and Charbonnier, J-M and Deconinck, H},
  booktitle={28th Fluid Dynamics Conference},
  pages={2023},
  year={1997}
}

@article{roy2003methodology,
  title={Methodology for turbulence model validation: application to hypersonic flows},
  author={Roy, Christopher J and Blottner, Frederick G},
  journal={Journal of spacecraft and rockets},
  volume={40},
  number={3},
  pages={313--325},
  year={2003}
}

@article{rumsey2010compressibility,
  title={Compressibility considerations for kw turbulence models in hypersonic boundary-layer applications},
  author={Rumsey, Christopher L},
  journal={Journal of Spacecraft and Rockets},
  volume={47},
  number={1},
  pages={11--20},
  year={2010}
}

@article{schmisseur2015hypersonics,
  title={Hypersonics into the 21st century: A perspective on AFOSR-sponsored research in aerothermodynamics},
  author={Schmisseur, John D},
  journal={Progress in Aerospace Sciences},
  volume={72},
  pages={3--16},
  year={2015},
  publisher={Elsevier}
}


@inproceedings{wilcox1991progress,
  title={Progress in hypersonic turbulence modeling},
  author={Wilcox, David},
  booktitle={22nd Fluid Dynamics, Plasma Dynamics and Lasers Conference},
  pages={1785},
  year={1991}
}


@inproceedings{gnoffo2011uncertainty,
  title={Uncertainty assessments of 2D and axisymmetric hypersonic shock wave-turbulent boundary layer interaction simulations at compression corners},
  author={Gnoffo, Peter and Berry, Scott and Van Norman, John},
  booktitle={42nd AIAA thermophysics conference},
  pages={3142},
  year={2011}
}

@inproceedings{brown2011shock,
  title={Shock wave impingement on boundary layers at hypersonic speeds: computational analysis and uncertainty},
  author={Brown, James},
  booktitle={42nd AIAA Thermophysics Conference},
  pages={3143},
  year={2011}
}

@article{gnoffo2013uncertainty,
  title={Uncertainty assessments of hypersonic shock wave-turbulent boundary-layer interactions at compression corners},
  author={Gnoffo, Peter A and Berry, Scott A and Van Norman, John W},
  journal={Journal of Spacecraft and Rockets},
  volume={50},
  number={1},
  pages={69--95},
  year={2013}
}

@article{goldberg2000hypersonic,
  title={Hypersonic flow predictions using linear and nonlinear turbulence closures},
  author={Goldberg, U and Batten, P and Palaniswamy, S and Chakravarthy, S and Peroomian, O},
  journal={Journal of Aircraft},
  volume={37},
  number={4},
  pages={671--675},
  year={2000}
}

@article{goldberg2001hypersonic,
  title={Hypersonic flow heat transfer prediction using single equation turbulence models},
  author={Goldberg, U},
  journal={J. Heat Transfer},
  volume={123},
  number={1},
  pages={65--69},
  year={2001}
}

@article{brown2013hypersonic,
  title={Hypersonic shock wave impingement on turbulent boundary layers: computational analysis and uncertainty},
  author={Brown, James L},
  journal={Journal of Spacecraft and Rockets},
  volume={50},
  number={1},
  pages={96--123},
  year={2013}
}


@techreport{marvin2013experimental,
  title={Experimental database with baseline CFD solutions: 2-D and axisymmetric hypersonic shock-wave/turbulent-boundary-layer interactions},
  author={Marvin, Joseph G and Brown, James L and Gnoffo, Peter A},
  year={2013}
}

@article{schulein2006skin,
  title={Skin friction and heat flux measurements in shock/boundary layer interaction flows},
  author={Sch{\"u}lein, Erich},
  journal={AIAA journal},
  volume={44},
  number={8},
  pages={1732--1741},
  year={2006}
}

@inproceedings{rumsey2015recent,
  title={Recent developments on the turbulence modeling resource website},
  author={Rumsey, Christopher L},
  booktitle={22nd AIAA Computational Fluid Dynamics Conference},
  pages={2927},
  year={2015}
}

@inproceedings{holden2010experimental,
  title={Experimental studies of shock wave/turbulent boundary layer interaction in high Reynolds number supersonic and hypersonic flows to evaluate the performance of CFD codes},
  author={Holden, Michael and Wadhams, Timothy and MacLean, Matthew and Mundy, Erik},
  booktitle={40th fluid dynamics conference and exhibit},
  pages={4468},
  year={2010}
}

@article{raje2021anisotropic,
  title={Anisotropic SST turbulence model for shock-boundary layer interaction},
  author={Raje, Pratikkumar and Sinha, Krishnendu},
  journal={Computers \& Fluids},
  volume={228},
  pages={105072},
  year={2021},
  publisher={Elsevier}
}

@inproceedings{holden2012review,
  title={Review of basic research and development programs conducted in the lens facilities in hypersonic flows},
  author={Holden, Michael and Wadhams, Timothy and MacLean, Matthew and Dufrene, Aaron and Mundy, Erik and Marineau, Eric},
  booktitle={50th AIAA Aerospace Sciences Meeting including the New Horizons Forum and Aerospace Exposition},
  pages={469},
  year={2012}
}

@inproceedings{waligura2022investigation,
  title={Investigation of spalart-allmaras turbulence model modifications for hypersonic flows utilizing output-based grid adaptation},
  author={Waligura, Carter J and Couchman, Benjamin L and Galbraith, Marshall C and Allmaras, Steven R and Harris, Wesley L},
  booktitle={AIAA SciTech 2022 Forum},
  pages={0587},
  year={2022}
}

@article{pasha2012simulation,
  title={Simulation of hypersonic shock/turbulent boundary-layer interactions using shock-unsteadiness model},
  author={Pasha, Amjad A and Sinha, Krishnendu},
  journal={Journal of Propulsion and Power},
  volume={28},
  number={1},
  pages={46--60},
  year={2012}
}

@article{xiao2007modeling,
  title={Modeling scramjet flows with variable turbulent Prandtl and Schmidt numbers},
  author={Xiao, Xudong and Hassan, Hassan A and Baurle, Robert A},
  journal={AIAA journal},
  volume={45},
  number={6},
  pages={1415--1423},
  year={2007}
}

@article{pecnik2012reynolds,
  title={Reynolds-averaged Navier-Stokes simulations of the HyShot II scramjet},
  author={Pecnik, Ren{\'e} and Terrapon, Vincent E and Ham, Frank and Iaccarino, Gianluca and Pitsch, Heinz},
  journal={AIAA journal},
  volume={50},
  number={8},
  pages={1717--1732},
  year={2012}
}

@inproceedings{georgiadis2013recalibration,
  title={Recalibration of the shear stress transport model to improve calculation of shock separated flows},
  author={Georgiadis, Nicholas and Yoder, Dennis},
  booktitle={51st AIAA Aerospace Sciences Meeting Including the New Horizons Forum and Aerospace Exposition},
  pages={685},
  year={2013}
}

@inproceedings{coakley1992turbulence,
  title={Turbulence modeling for high speed flows},
  author={Coakley, T and Huang, P},
  booktitle={30th Aerospace Sciences Meeting and Exhibit},
  pages={436},
  year={1992}
}

@article{zhang2022application,
  title={Application of linear and nonlinear two-equation turbulence models in hypersonic flows},
  author={Zhang, Haoyuan and Craft, Timothy and Iacovides, Hector},
  journal={AIAA Journal},
  volume={60},
  number={6},
  pages={3472--3486},
  year={2022},
  publisher={American Institute of Aeronautics and Astronautics}
}

@article{zhao2019uncertainty,
  title={Uncertainty and sensitivity analysis of SST turbulence model on hypersonic flow heat transfer},
  author={Zhao, Yatian and Yan, Chao and Wang, Xiaoyong and Liu, Hongkang and Zhang, Wei},
  journal={International Journal of Heat and Mass Transfer},
  volume={136},
  pages={808--820},
  year={2019},
  publisher={Elsevier}
}

@article{huang2019assessment,
  title={Assessment of turbulence models in a hypersonic cold-wall turbulent boundary layer},
  author={Huang, Junji and Bretzke, Jorge-Valentino and Duan, Lian},
  journal={Fluids},
  volume={4},
  number={1},
  pages={37},
  year={2019},
  publisher={MDPI}
}

@article{lagares2021turbulence,
  title={Turbulence modeling in hypersonic turbulent boundary layers subject to convex wall curvature},
  author={Lagares-Nieves, Christian J and Santiago, Jean and Araya, Guillermo},
  journal={AIAA Journal},
  volume={59},
  number={12},
  pages={4935--4954},
  year={2021},
  publisher={American Institute of Aeronautics and Astronautics}
}

@article{paciorri1998exploring,
  title={Exploring the validity of the Spalart-Allmaras turbulence model for hypersonic flows},
  author={Paciorri, Renato and Dieudonn{\'e}, Walter and Degrez, G{\'e}rard and Charbonnier, J-M and Deconinck, Herman},
  journal={Journal of Spacecraft and Rockets},
  volume={35},
  number={2},
  pages={121--126},
  year={1998}
}

@article{coratekin2004performance,
  title={Performance of upwind schemes and turbulence models in hypersonic flows},
  author={Coratekin, Turan and Van Keuk, J{\"o}rn and Ballmann, Josef},
  journal={AIAA journal},
  volume={42},
  number={5},
  pages={945--957},
  year={2004}
}

@article{chowdhary2022calibrating,
  title={Calibrating hypersonic turbulence flow models with the HIFiRE-1 experiment using data-driven machine-learned models},
  author={Chowdhary, Kenny and Hoang, Chi and Lee, Kookjin and Ray, Jaideep and Weirs, V Gregory and Carnes, Brian},
  journal={Computer Methods in Applied Mechanics and Engineering},
  volume={401},
  pages={115396},
  year={2022},
  publisher={Elsevier}
}

@inproceedings{yoon2007computational,
  title={Computational challenges in hypersonic flow simulations},
  author={Yoon, Seokkwan and Gnoffo, Peter and White, Jeffery and Thomas, James},
  booktitle={39th AIAA Thermophysics Conference},
  pages={4265},
  year={2007}
}

@article{sarma2000physico,
  title={Physico--chemical modelling in hypersonic flow simulation},
  author={Sarma, GSR},
  journal={Progress in Aerospace Sciences},
  volume={36},
  number={3-4},
  pages={281--349},
  year={2000},
  publisher={Elsevier}
}

@book{anderson1989hypersonic,
  title={Hypersonic and high temperature gas dynamics},
  author={Anderson, John David},
  year={1989},
  publisher={Aiaa}
}

@inproceedings{coakley1990assessment,
  title={An assessment and application of turbulence models for hypersonic flows},
  author={Coakley, TJ and Viegas, JR and Huang, PG and Rubesin, MW},
  booktitle={National Aero-Space Plane Technology Symposium},
  number={PAPER-106},
  year={1990}
}

@inproceedings{rubesin1989turbulence,
  title={Turbulence modeling for aerodynamic flows},
  author={RUBESIN, MORRIS},
  booktitle={27th Aerospace Sciences Meeting},
  pages={606},
  year={1989}
}

@article{candler2015advances,
  title={Advances in computational fluid dynamics methods for hypersonic flows},
  author={Candler, Graham V and Subbareddy, Pramod K and Brock, Joseph M},
  journal={Journal of Spacecraft and Rockets},
  volume={52},
  number={1},
  pages={17--28},
  year={2015},
  publisher={American Institute of Aeronautics and Astronautics}
}

@article{li2021bayesian,
  title={Bayesian model evaluation of three k--$\omega$ turbulence models for hypersonic shock wave--boundary layer interaction flows},
  author={Li, Jin-ping and Zeng, Fan-zhi and Chen, Shu-sheng and Zhang, Kai-ling and Yan, Chao},
  journal={Acta Astronautica},
  volume={189},
  pages={143--157},
  year={2021},
  publisher={Elsevier}
}

@inproceedings{candler2015next,
  title={Next-generation CFD for hypersonic and aerothermal flows},
  author={Candler, Graham V},
  booktitle={22nd AIAA Computational Fluid Dynamics Conference},
  pages={3048},
  year={2015}
}

@inproceedings{bardina1992two,
  title={Two-equation turbulence modeling for 3-d hypersonic flows},
  author={Bardina, J and Coakley, T and Marvin, J},
  booktitle={AlAA 4th International Aerospace Planes Conference},
  pages={5064},
  year={1992}
}

@article{nguyen2006modeling,
  title={Modeling and simulation of turbulent reacting flow around a hypersonic space probe},
  author={Nguyen-Bui, NT-H and Duffa, G},
  journal={Journal of spacecraft and rockets},
  volume={43},
  number={4},
  pages={919--923},
  year={2006}
}

@article{roy2019turbulent,
  title={Turbulent heat flux model for hypersonic shock--boundary layer interaction},
  author={Roy, Subhajit and Sinha, Krishnendu},
  journal={AIAA Journal},
  volume={57},
  number={8},
  pages={3624--3629},
  year={2019},
  publisher={American Institute of Aeronautics and Astronautics}
}

@inproceedings{erb2018investigation,
  title={Investigation of turbulence model uncertainty for supersonic/hypersonic shock wave-boundary layer interaction predictions},
  author={Erb, Aaron J and Hosder, Serhat},
  booktitle={22nd AIAA International Space Planes and Hypersonics Systems and Technologies Conference},
  pages={5195},
  year={2018}
}

@article{candler2019rate,
  title={Rate effects in hypersonic flows},
  author={Candler, Graham V},
  journal={Annual Review of Fluid Mechanics},
  volume={51},
  number={1},
  pages={379--402},
  year={2019},
  publisher={Annual Reviews}
}

@article{hu1995turbulent,
  title={Turbulent flow in supersonic and hypersonic nozzles},
  author={Hu, Jiasen and Rizzi, Arthur},
  journal={AIAA journal},
  volume={33},
  number={9},
  pages={1634--1640},
  year={1995}
}

@article{reddy2009hypersonic,
  title={Hypersonic turbulent flow simulation of Fire II reentry vehicle afterbody},
  author={Reddy, D Siva K and Sinha, Krishnendu},
  journal={Journal of Spacecraft and Rockets},
  volume={46},
  number={4},
  pages={745--757},
  year={2009}
}

@inproceedings{bardina1994three,
  title={Three-dimensional Navier-Stokes method with two-equation turbulence models for efficient numerical simulation of hypersonic flows},
  author={Bardina, J},
  booktitle={30th Joint Propulsion Conference and Exhibit},
  pages={2950},
  year={1994}
}

@inproceedings{nicholson2021simulation,
  title={Simulation and modeling of hypersonic turbulent boundary layers subject to adverse pressure gradients due to streamline curvature},
  author={Nicholson, Gary and Huang, Junji and Duan, Lian and Choudhari, Meelan M},
  booktitle={AIAA Aviation 2021 Forum},
  pages={2891},
  year={2021}
}

@article{yancheng2012evaluation,
  title={Evaluation of Turbulence Models in Predicting Hypersonic and Subsonic Base Flows Using Grid Adaptation Techniques},
  author={Yancheng, YOU and Buanga, Bj{\"o}rn and Hannemann, Volker and Luedeke, Heinrich},
  journal={Chinese Journal of Aeronautics},
  volume={25},
  number={3},
  pages={325--334},
  year={2012},
  publisher={Elsevier}
}


@inproceedings{huang2020simulation,
  title={Simulation and modeling of cold-wall hypersonic turbulent boundary layers on flat plate},
  author={Huang, Junji and Nicholson, Gary L and Duan, Lian and Choudhari, Meelan M and Bowersox, Rodney D},
  booktitle={AIAA Scitech 2020 Forum},
  pages={0571},
  year={2020}
}

@article{ng1989turbulence,
  title={Turbulence modeling in a hypersonic inlet},
  author={Ng, Wing-Fai and Ajmani, K and Taylor III, AC},
  journal={AIAA journal},
  volume={27},
  number={10},
  pages={1354--1360},
  year={1989}
}

@inproceedings{bardina1994three-1,
  title={Three-Dimensional Navier-Stokes Simulations with Two-Equation Turbulence Models of Intersecting Shock-Waves/Turbulent Boundary Layer at Mach 8.3},
  author={Bardina, Jorge E and Coakley, Thomas J},
  booktitle={Applied Aerodynamics Conference},
  number={NASA-CR-201979},
  year={1994}
}

@article{yentsch2014performance,
  title={Performance of turbulence modeling in simulation of the HIFiRE-1 flight test},
  author={Yentsch, Robert J and Gaitonde, Datta V and Kimmel, Roger},
  journal={Journal of Spacecraft and Rockets},
  volume={51},
  number={1},
  pages={117--127},
  year={2014},
  publisher={American Institute of Aeronautics and Astronautics}
}

@article{smith1996prediction,
  title={Prediction of hypersonic shock-wave/turbulent boundary-layer interactions},
  author={Smith, Brian R},
  journal={Journal of spacecraft and rockets},
  volume={33},
  number={5},
  pages={614--619},
  year={1996}
}

@inproceedings{jie2011stress,
  title={Stress limiter consideration for k-omega turbulence models in shock-wave/turbulent boundary-layer interactions in supersonic and hypersonic flows},
  author={Jie, Tan and Jie, Jin},
  booktitle={20th AIAA Computational Fluid Dynamics Conference},
  pages={3980},
  year={2011}
}

@inproceedings{georgiadis2014turbulence,
  title={Turbulence model effects on RANS simulations of the HIFiRE flight 2 ground test configurations},
  author={Georgiadis, Nicholas J and Mankbadi, Mina R and Vyas, Manan A},
  booktitle={52nd Aerospace Sciences Meeting},
  pages={0624},
  year={2014}
}

@article{zhang2010turbulence,
  title={Turbulence models for accurate aerothermal prediction in hypersonic flows},
  author={Zhang, Xiang-Hong and Wu, Yi-Zao and Wang, Jiang-Feng},
  journal={Modern Physics Letters B},
  volume={24},
  number={13},
  pages={1345--1348},
  year={2010},
  publisher={World Scientific}
}

@inproceedings{aiken2022assessment,
  title={Assessment of Reynolds Averaged Navier-Stokes models for a hypersonic cold-wall turbulent boundary layer},
  author={Aiken, Timothy T and Boyd, Iain D and Duan, Lian and Huang, Junji},
  booktitle={AIAA SciTech 2022 Forum},
  pages={0586},
  year={2022}
}

@article{kral1998recent,
  title={Recent experience with different turbulence models applied to the calculation of flow over aircraft components},
  author={Kral, LD},
  journal={Progress in Aerospace Sciences},
  volume={34},
  number={7-8},
  pages={481--541},
  year={1998},
  publisher={Elsevier}
}

@article{danis2022compressibility,
  title={Compressibility correction to k- $\omega$ models for hypersonic turbulent boundary layers},
  author={Danis, Mustafa E and Durbin, Paul},
  journal={AIAA Journal},
  volume={60},
  number={11},
  pages={6225--6234},
  year={2022},
  publisher={American Institute of Aeronautics and Astronautics}
}

@incollection{huang1993calculations,
  title={Calculations of supersonic and hypersonic flows using compressible wall functions},
  author={Huang, PG and Coakley, TJ},
  booktitle={Engineering Turbulence Modelling and Experiments},
  pages={731--739},
  year={1993},
  publisher={Elsevier}
}

@article{knight2017assessment,
  title={Assessment of predictive capabilities for aerodynamic heating in hypersonic flow},
  author={Knight, Doyle and Chazot, Olivier and Austin, Joanna and Badr, Mohammad Ali and Candler, Graham and Celik, Bayram and de Rosa, Donato and Donelli, Raffaele and Komives, Jeffrey and Lani, Andrea and others},
  journal={Progress in Aerospace Sciences},
  volume={90},
  pages={39--53},
  year={2017},
  publisher={Elsevier}
}

@article{xiao2007role,
  title={Role of turbulent Prandtl numbers on heat flux at hypersonic Mach numbers},
  author={Xiao, Xudong and Hassan, HA and Edwards, JR and Gaffney Jr, RL},
  journal={AIAA journal},
  volume={45},
  number={4},
  pages={806--813},
  year={2007}
}

@article{hoskin2024discontinuous,
  title={Discontinuous Galerkin methods for hypersonic flows},
  author={Hoskin, Dominique S and Van Heyningen, R Loek and Nguyen, Ngoc Cuong and Vila-P{\'e}rez, Jordi and Harris, Wesley L and Peraire, Jaime},
  journal={Progress in Aerospace Sciences},
  volume={146},
  pages={100999},
  year={2024},
  publisher={Elsevier}
}

@inproceedings{holden2006historical,
  title={Historical review of experimental studies and prediction methods to describe laminar and turbulent shock wave/boundary layer interactions in hypersonic flows},
  author={Holden, Michael},
  booktitle={44th AIAA Aerospace Sciences Meeting and Exhibit},
  pages={494},
  year={2006}
}

@book{babinsky2011shock,
  title={Shock wave-boundary-layer interactions},
  author={Babinsky, Holger and Harvey, John K},
  volume={32},
  year={2011},
  publisher={Cambridge University Press}
}

@article{gaitonde2015progress,
  title={Progress in shock wave/boundary layer interactions},
  author={Gaitonde, Datta V},
  journal={Progress in Aerospace Sciences},
  volume={72},
  pages={80--99},
  year={2015},
  publisher={Elsevier}
}

@article{gaitonde2023dynamics,
  title={Dynamics of three-dimensional shock-wave/boundary-layer interactions},
  author={Gaitonde, Datta V and Adler, Michael C},
  journal={Annual Review of Fluid Mechanics},
  volume={55},
  number={1},
  pages={291--321},
  year={2023},
  publisher={Annual Reviews}
}

@article{shyy1997compressibility,
  title={Compressibility effects in modeling complex turbulent flows},
  author={Shyy, Wei and Krishnamurty, Venkata S},
  journal={Progress in aerospace sciences},
  volume={33},
  number={9-10},
  pages={587--645},
  year={1997},
  publisher={Elsevier}
}

@book{gatski2013compressibility,
  title={Compressibility, turbulence and high speed flow},
  author={Gatski, Thomas B and Bonnet, Jean-Paul},
  year={2013},
  publisher={Academic Press}
}

@article{catris2000density,
  title={Density corrections for turbulence models},
  author={Catris, St{\'e}phane and Aupoix, Bertrand},
  journal={Aerospace Science and Technology},
  volume={4},
  number={1},
  pages={1--11},
  year={2000},
  publisher={Elsevier}
}

@article{dai2022influence,
  title={Influence of high temperature non-equilibrium effects on Mach 12 scramjet inlet},
  author={Dai, Chunliang and Sun, Bo and Zhou, Shengbing and Zhuo, Changfei and Zhou, Changsheng and Yue, Lianjie},
  journal={Acta Astronautica},
  volume={193},
  pages={237--254},
  year={2022},
  publisher={Elsevier}
}

@article{barth2015effects,
  title={Effects of hydrogen fuel injection in a Mach 12 scramjet inlet},
  author={Barth, James E and Wheatley, Vincent and Smart, Michael K},
  journal={AIAA Journal},
  volume={53},
  number={10},
  pages={2907--2919},
  year={2015},
  publisher={American Institute of Aeronautics and Astronautics}
}

@article{dai2022numerical,
  title={Numerical study of high temperature non-equilibrium effects of double-wedge in hypervelocity flow},
  author={Dai, Chunliang and Sun, Bo and Zhuo, Changfei and Zhou, Shengbing and Zhou, Changsheng and Yue, Lianjie},
  journal={Aerospace Science and Technology},
  volume={124},
  pages={107526},
  year={2022},
  publisher={Elsevier}
}

@article{sciacovelli2023priori,
  title={A priori tests of turbulence models for compressible flows},
  author={Sciacovelli, Luca and Cannici, Aron and Passiatore, Donatella and Cinnella, Paola},
  journal={International Journal of Numerical Methods for Heat \& Fluid Flow},
  year={2023},
  publisher={Emerald Publishing Limited}
}

@article{chen2024improved,
  title={An improved Baldwin--Lomax algebraic wall model for high-speed canonical turbulent boundary layers using established scalings},
  author={Chen, Xianliang and Gan, Jianping and Fu, Lin},
  journal={Journal of Fluid Mechanics},
  volume={987},
  pages={A7},
  year={2024},
  publisher={Cambridge University Press}
}

@article{wilcox1992dilatation,
  title={Dilatation-dissipation corrections for advanced turbulence models},
  author={Wilcox, David C},
  journal={AIAA journal},
  volume={30},
  number={11},
  pages={2639--2646},
  year={1992}
}

@article{urzay2018supersonic,
  title={Supersonic combustion in air-breathing propulsion systems for hypersonic flight},
  author={Urzay, Javier},
  journal={Annual Review of Fluid Mechanics},
  volume={50},
  number={1},
  pages={593--627},
  year={2018},
  publisher={Annual Reviews}
}

@article{urzay2021engineering,
  title={Engineering aspects of hypersonic turbulent flows at suborbital enthalpies},
  author={Urzay, J. and Di Renzo, M.},
  journal={Annual Research Briefs, Center for Turbulence Research},
  pages={7--32},
  year={2021}
}

@article{sarma2000physico,
  title={Physico--chemical modelling in hypersonic flow simulation},
  author={Sarma, GSR},
  journal={Progress in Aerospace Sciences},
  volume={36},
  number={3-4},
  pages={281--349},
  year={2000},
  publisher={Elsevier}
}

@inproceedings{molchanov2013three,
  title={Three-equation k-$\varepsilon$-Vn turbulence model for high-speed flows},
  author={Molchanov, Alexander M},
  booktitle={43rd AIAA Fluid Dynamics Conference},
  pages={3181},
  year={2013}
}

@article{duraisamy2019turbulence,
  title={Turbulence modeling in the age of data},
  author={Duraisamy, Karthik and Iaccarino, Gianluca and Xiao, Heng},
  journal={Annual review of fluid mechanics},
  volume={51},
  number={1},
  pages={357--377},
  year={2019},
  publisher={Annual Reviews}
}

@book{wilcox1998turbulence,
  title={Turbulence modeling for CFD},
  author={Wilcox, David C and others},
  volume={2},
  year={1998},
  publisher={DCW industries La Canada, CA}
}

@article{dolling2001fifty,
  title={Fifty years of shock-wave/boundary-layer interaction research: what next?},
  author={Dolling, David S},
  journal={AIAA journal},
  volume={39},
  number={8},
  pages={1517--1531},
  year={2001}
}

@inproceedings{zhang2015turbulence,
  title={Turbulence model modification for fake amplification of Turbulence Kinetic Energy by Shock-Turbulence Interation},
  author={Zhang, Zhichao and Gao, Zhenxun and Jiang, Chongwen and Lee, Chunhian},
  booktitle={51st AIAA/SAE/ASEE Joint Propulsion Conference},
  pages={4205},
  year={2015}
}

@article{lee1997interaction,
  title={Interaction of isotropic turbulence with shock waves: effect of shock strength},
  author={Lee, Sangsan and Lele, Sanjiva K and Moin, Parviz},
  journal={Journal of Fluid Mechanics},
  volume={340},
  pages={225--247},
  year={1997},
  publisher={Cambridge University Press}
}

@conference{KaWi95,
	author = {M Kandula and D Wilcox},
	booktitle = {Fluid Dynamics Conference},
	doi = {10.2514/6.1995-2317},
	eprint = {https://arc.aiaa.org/doi/pdf/10.2514/6.1995-2317},
	title = {An examination of k-omega turbulence model for boundary layers, free shear layers and separated flows},
    year = {1995},
	url = {https://arc.aiaa.org/doi/abs/10.2514/6.1995-2317},
	bdsk-url-1 = {https://arc.aiaa.org/doi/abs/10.2514/6.1995-2317},
	bdsk-url-2 = {https://doi.org/10.2514/6.1995-2317}}


@article{menter1994two,
  title={Two-equation eddy-viscosity turbulence models for engineering applications},
  author={Menter, Florian R},
  journal={AIAA journal},
  volume={32},
  number={8},
  pages={1598--1605},
  year={1994}
}

@incollection{steelant2002effect,
  title={Effect of a compressibility correction on different turbulence models},
  author={Steelant, Johan},
  booktitle={Engineering Turbulence Modelling and Experiments 5},
  pages={207--216},
  year={2002},
  publisher={Elsevier}
}

@article{huang1994turbulence,
  title={Turbulence models for compressible boundary layers},
  author={Huang, PG and Bradshaw, P and Coakley, TJ},
  journal={AIAA journal},
  volume={32},
  number={4},
  pages={735--740},
  year={1994}
}

@article{duan2011direct,
  title={Direct numerical simulation of hypersonic turbulent boundary layers. Part 3. Effect of Mach number},
  author={Duan, Lian and Beekman, I and Martin, MP},
  journal={Journal of Fluid Mechanics},
  volume={672},
  pages={245--267},
  year={2011},
  publisher={Cambridge University Press}
}

@article{rose1973ratio,
  title={Ratio of Reynolds shear stress to turbulence kinetic energy in a boundary layer},
  author={Rose, William C and Murphy, John D},
  journal={Physics of Fluids},
  volume={16},
  number={6},
  pages={935--937},
  year={1973}
}

@article{pope1975more,
  title={A more general effective-viscosity hypothesis},
  author={Pope, Stephen B},
  journal={Journal of Fluid Mechanics},
  volume={72},
  number={2},
  pages={331--340},
  year={1975},
  publisher={Cambridge University Press}
}

@article{raje2016physically,
  title={A physically consistent and numerically robust k-$\epsilon$ model for computing turbulent flows with shock waves},
  author={Raje, Pratikkumar and Sinha, Krishnendu},
  journal={Computers \& Fluids},
  volume={136},
  pages={35--47},
  year={2016},
  publisher={Elsevier}
}

@inproceedings{rodi1976new,
  title={A new algebraic relation for calculating the Reynolds stresses},
  author={Rodi, W},
  booktitle={Gesellschaft Angewandte Mathematik und Mechanik Workshop Paris France},
  volume={56},
  pages={219},
  year={1976}
}

@article{craft1996development,
  title={Development and application of a cubic eddy-viscosity model of turbulence},
  author={Craft, TJ and Launder, BE and Suga, K},
  journal={International Journal of Heat and Fluid Flow},
  volume={17},
  number={2},
  pages={108--115},
  year={1996},
  publisher={Elsevier}
}

@article{gatski2000nonlinear,
  title={Nonlinear eddy viscosity and algebraic stress models for solving complex turbulent flows},
  author={Gatski, TB and Jongen, T},
  journal={Progress in Aerospace Sciences},
  volume={36},
  number={8},
  pages={655--682},
  year={2000},
  publisher={Elsevier}
}

@inproceedings{lindblad1998prediction,
  title={A prediction method for high speed turbulent separated flows with experimental verification},
  author={Lindblad, I and Wallin, S and Johansson, A and Friedrich, R and Lechner, R and Krogmann, P and Schuelein, E and Courty, J-C and Ravachol, M and Giordano, D},
  booktitle={29th AIAA, Fluid Dynamics Conference},
  pages={2547},
  year={1998}
}

@article{wallin2000explicit,
  title={An explicit algebraic Reynolds stress model for incompressible and compressible turbulent flows},
  author={Wallin, Stefan and Johansson, Arne V},
  journal={Journal of fluid mechanics},
  volume={403},
  pages={89--132},
  year={2000},
  publisher={Cambridge University Press}
}

@article{vemula2020explicit,
  title={Explicit algebraic Reynolds stress model for shock-dominated flows},
  author={Vemula, Jagadish Babu and Sinha, Krishnendu},
  journal={International Journal of Heat and Fluid Flow},
  volume={85},
  pages={108680},
  year={2020},
  publisher={Elsevier}
}
 @article{Vemula_Sinha_2017, title={Reynolds stress models applied to canonical shock-turbulence interaction}, volume={18}, ISSN={1468-5248}, DOI={10.1080/14685248.2017.1317923}, number={7}, journal={Journal of Turbulence}, author={Vemula, Jagadish Babu and Sinha, Krishnendu}, year={2017}, month=jul, pages={653–687}, language={en} }


@article{gatski1993explicit,
  title={On explicit algebraic stress models for complex turbulent flows},
  author={Gatski, Thomas B and Speziale, Charles G},
  journal={Journal of fluid Mechanics},
  volume={254},
  pages={59--78},
  year={1993},
  publisher={Cambridge University Press}
}

@article{launder1975progress,
  title={Progress in the development of a Reynolds-stress turbulence closure},
  author={Launder, Brian Edward and Reece, G Jr and Rodi, W},
  journal={Journal of fluid mechanics},
  volume={68},
  number={3},
  pages={537--566},
  year={1975},
  publisher={Cambridge University Press}
}

@article{rotta1951statistische,
  title={Statistische theorie nichthomogener turbulenz},
  author={Rotta, JC},
  journal={Zeitschrift f{\"u}r Physik},
  volume={129},
  pages={547--572},
  year={1951},
  publisher={Springer}
}

@article{jongen1998general,
  title={General explicit algebraic stress relations and best approximation for three-dimensional flows},
  author={Jongen, T and Gatski, TB},
  journal={International Journal of Engineering Science},
  volume={36},
  number={7-8},
  pages={739--763},
  year={1998},
  publisher={Elsevier}
}

@book{boussinesq1877essai,
  title={Essai sur la th{\'e}orie des eaux courantes},
  author={Boussinesq, Jean},
  year={1877},
  publisher={Imprimerie nationale}
}


@article{prandtl1925,
author = {Prandtl, L.},
title = {7. Bericht über Untersuchungen zur ausgebildeten Turbulenz},
journal = {ZAMM - Journal of Applied Mathematics and Mechanics / Zeitschrift für Angewandte Mathematik und Mechanik},
volume = {5},
number = {2},
pages = {136-139},
doi = {https://doi.org/10.1002/zamm.19250050212},
url = {https://onlinelibrary.wiley.com/doi/abs/10.1002/zamm.19250050212},
eprint = {https://onlinelibrary.wiley.com/doi/pdf/10.1002/zamm.19250050212},
year = {1925}
}

@article{chou1945velocity,
  title={On velocity correlations and the solutions of the equations of turbulent fluctuation},
  author={Chou, Pei-Yuan},
  journal={Quarterly of applied mathematics},
  volume={3},
  number={1},
  pages={38--54},
  year={1945}
}

@inproceedings{kolmogorov1941equations,
  title={Equations of turbulent motion in an incompressible fluid},
  author={Kolmogorov, Andrej Nikolaevich},
  booktitle={Dokl. Akad. Nauk SSSR},
  volume={30},
  pages={299--303},
  year={1941}
}

@article{sarkar1991analysis,
  title={The analysis and modelling of dilatational terms in compressible turbulence},
  author={Sarkar, Sutanu and Erlebacher, Gordon and Hussaini, M Yousuff and Kreiss, Heinz Otto},
  journal={Journal of Fluid Mechanics},
  volume={227},
  pages={473--493},
  year={1991},
  publisher={Cambridge University Press}
}

@article{settles1994hypersonic,
  title={Hypersonic shock/boundary-layer interaction database: new and corrected data},
  author={Settles, Gary S and Dodson, Lori J},
  journal={Pennsylvania State Univ. Report},
  year={1994}
}

@article{zhang2018direct,
  title={Direct numerical simulation database for supersonic and hypersonic turbulent boundary layers},
  author={Zhang, Chao and Duan, Lian and Choudhari, Meelan M},
  journal={AIAA journal},
  volume={56},
  number={11},
  pages={4297--4311},
  year={2018},
  publisher={American Institute of Aeronautics and Astronautics}
}

@article{murray2013experimental,
  title={Experimental investigation of axisymmetric hypersonic shock-wave/turbulent-boundary-layer interactions},
  author={Murray, N and Hillier, R and Williams, S},
  journal={Journal of Fluid Mechanics},
  volume={714},
  pages={152--189},
  year={2013},
  publisher={Cambridge University Press}
}

@phdthesis{williams2005three,
  title={Three-dimensional separation of a hypersonic boundary layer},
  author={Williams, Simon},
  year={2005},
  school={Imperial College London}
}

@phdthesis{murray2007three,
  title={Three-dimensional turbulent shock-wave: boundary-layer interactions in hypersonic flows},
  author={Murray, Neil Paul},
  year={2007},
  school={Imperial College London (University of London)}
}

@phdthesis{coleman1973hypersonic,
  title={Hypersonic turbulent boundary layer studies},
  author={Coleman, Graham Trevor},
  year={1973},
  school={Imperial College London}
}

@article{coleman1972heat,
  title={Heat transfer from hypersonic turbulent flow at a wedge compression corner},
  author={Coleman, GT and Stollery, JL},
  journal={Journal of Fluid Mechanics},
  volume={56},
  number={4},
  pages={741--752},
  year={1972},
  publisher={Cambridge University Press}
}

@article{elfstrom1972turbulent,
  title={Turbulent hypersonic flow at a wedge-compression corner},
  author={Elfstrom, GM},
  journal={Journal of fluid Mechanics},
  volume={53},
  number={1},
  pages={113--127},
  year={1972},
  publisher={Cambridge University Press}
}

@article{kussoy1991documentation,
  title={Documentation of two-and three-dimensional shock-wave/turbulent-boundary-layer interaction flows at Mach 8.2},
  author={Kussoy, Marvin I and Horstman, KC},
  journal={NASA Ames Research Center Technical Report},
  year={1991}
}
@techreport{parish2024report,
  title={{Data-driven closure modeling for
hypersonic turbulent flows}},
  author={Parish, Eric and Barone, Matthew and Ching, David and Jordan, Cyrus and Miller, Nathan and Nicholson, Gary and Gitushi, Kevin and Beresh, Steven and Gupta, Niloy and Duraisamy, Karthik},
  year={2024},
  institution={Sandia National Laboratories}
}
@techreport{holden1988studies,
  title={Studies of the structure of attached and separated regions of viscous/inviscid interaction and the effects of combined surface roughness and blowing in high-Reynolds-number hypersonic flows. Final report, 1 August 1985-1 June 1988},
  author={Holden, MS and Bergman, R and Harvey, J and Duryea, G and Moselle, J},
  year={1988},
  institution={Calspan UB Research Center, Buffalo, NY (USA)}
}

@article{holden1986shock,
  title={Shock wave/turbulent boundary layer interaction in high-Reynolds number hypersonic flows},
  author={Holden, MS and Havener, AG and Lee, CH},
  journal={Calspan-University of Buffalo Research Centre, CUBRC-86681},
  year={1986}
}

@inproceedings{holden1991studies,
  title={Studies of the mean and unsteady structure of turbulent boundary layer separation in hypersonic flow},
  author={Holden, M},
  booktitle={22nd Fluid Dynamics, Plasma Dynamics and Lasers Conference},
  pages={1778},
  year={1991}
}

@book{kussoy1989documentation,
  title={Documentation of two-and three-dimensional hypersonic shock wave/turbulent boundary layer interaction flows},
  author={Kussoy, Marvin I},
  volume={101075},
  year={1989},
  publisher={National Aeronautics and Space Administration, Ames Research Center}
}

@article{volpiani2020effects,
  title={Effects of a nonadiabatic wall on hypersonic shock/boundary-layer interactions},
  author={Volpiani, Pedro S and Bernardini, Matteo and Larsson, Johan},
  journal={Physical Review Fluids},
  volume={5},
  number={1},
  pages={014602},
  year={2020},
  publisher={APS}
}

@inproceedings{volpiani2019using,
  title={Using large-eddy simulations to design a new hypersonic shock/boundary-layer interaction experiment},
  author={Volpiani, Pedro S and Wagner, Alexander and Bernardini, Matteo and Larsson, Johan},
  booktitle={AIAA Scitech 2019 Forum},
  pages={0098},
  year={2019}
}

@article{duan2011direct4,
  title={Direct numerical simulation of hypersonic turbulent boundary layers. Part 4. Effect of high enthalpy},
  author={Duan, Lian and Martin, MP},
  journal={Journal of Fluid Mechanics},
  volume={684},
  pages={25--59},
  year={2011},
  publisher={Cambridge University Press}
}


@article{morkovin1962effects,
  title={Effects of compressibility on turbulent flows},
  author={Morkovin, Mark V},
  journal={M{\'e}canique de la Turbulence},
  volume={367},
  number={380},
  pages={26},
  year={1962},
  publisher={CNRS Paris}
}

@article{passiatore2021finite,
  title={Finite-rate chemistry effects in turbulent hypersonic boundary layers: A direct numerical simulation study},
  author={Passiatore, Donatella and Sciacovelli, Luca and Cinnella, Paola and Pascazio, Giuseppe},
  journal={Physical Review Fluids},
  volume={6},
  number={5},
  pages={054604},
  year={2021},
  publisher={APS}
}


@article{zeman1990dilatation,
  title={Dilatation dissipation: the concept and application in modeling compressible mixing layers},
  author={Zeman, Otto},
  journal={Physics of Fluids A: Fluid Dynamics},
  volume={2},
  number={2},
  pages={178--188},
  year={1990},
  publisher={American Institute of Physics}
}

@phdthesis{kim2016non,
  title={Non-equilibrium effects on hypersonic turbulent boundary layers},
  author={Kim, Pilbum},
  year={2016},
  school={University of California, Los Angeles}
}

@inproceedings{baurle2004modeling,
  title={Modeling of high speed reacting flows: established practices and future challenges},
  author={Baurle, Robert},
  booktitle={42nd AIAA aerospace sciences meeting and exhibit},
  pages={267},
  year={2004}
}

@inproceedings{ebrahimi2004overview,
  title={An overview of computational fluid dynamics for application to advanced propulsion systems},
  author={Ebrahimi, Houshang},
  booktitle={37th AIAA Thermophysics Conference},
  pages={2370},
  year={2004}
}

@article{dang2022direct,
  title={Direct numerical simulation of compressible turbulence accelerated by graphics processing unit: An open-source high accuracy accelerated computational fluid dynamic software},
  author={Dang, Guanlin and Liu, Shiwei and Guo, Tongbiao and Duan, Junyi and Li, Xinliang},
  journal={Physics of Fluids},
  volume={34},
  number={12},
  year={2022},
  publisher={AIP Publishing}
}

@article{priebe2021turbulence,
  title={Turbulence in a hypersonic compression ramp flow},
  author={Priebe, Stephan and Mart{\'\i}n, M Pino},
  journal={Physical Review Fluids},
  volume={6},
  number={3},
  pages={034601},
  year={2021},
  publisher={APS}
}

@article{yu2023coherent,
  title={Coherent structures and turbulent model refinement in oblique shock/hypersonic turbulent boundary layer interactions},
  author={Yu, Ming and Sun, Dong and Zhou, QingQing and Liu, PengXin and Yuan, XianXu},
  journal={Physics of Fluids},
  volume={35},
  number={8},
  year={2023},
  publisher={AIP Publishing}
}


@article{helm2022large,
  title={Large eddy simulation of two separated hypersonic shock/turbulent boundary layer interactions},
  author={Helm, Clara M and Mart{\'\i}n, MP},
  journal={Physical Review Fluids},
  volume={7},
  number={7},
  pages={074601},
  year={2022},
  publisher={APS}
}

@article{zuo2023hypersonic,
  title={Hypersonic shock wave/turbulent boundary layer interaction over a compression ramp},
  author={Zuo, Feng-Yuan},
  journal={AIAA Journal},
  volume={61},
  number={4},
  pages={1579--1595},
  year={2023},
  publisher={American Institute of Aeronautics and Astronautics}
}

@article{zhang2022direct,
  title={Direct numerical simulation of shock wave/turbulent boundary layer interaction in a swept compression ramp at Mach 6},
  author={Zhang, Ji and Guo, Tongbiao and Dang, Guanlin and Li, Xinliang},
  journal={Physics of Fluids},
  volume={34},
  number={11},
  year={2022},
  publisher={AIP Publishing}
}

@article{guo2023amplification,
  title={Amplification of turbulent kinetic energy and temperature fluctuation in a hypersonic turbulent boundary layer over a compression ramp},
  author={Guo, Tongbiao and Zhang, Ji and Tong, Fulin and Li, Xinliang},
  journal={Physics of Fluids},
  volume={35},
  number={4},
  year={2023},
  publisher={AIP Publishing}
}

@article{chen2022wall,
  title={LES wall modeling for heat transfer at high speeds},
  author={Chen, Peng ES and Lv, Yu and Xu, Haosen HA and Shi, Yipeng and Yang, Xiang IA},
  journal={Physical Review Fluids},
  volume={7},
  number={1},
  pages={014608},
  year={2022},
  publisher={APS}
}

@article{fulin2023hypersonic,
  title={Hypersonic shock wave and turbulent boundary layer interaction in a sharp cone/flare model},
  author={Fulin, TONG and Junyi, DUAN and Jiang, LAI and Dong, SUN and Xianxu, YUAN},
  journal={Chinese Journal of Aeronautics},
  volume={36},
  number={3},
  pages={80--95},
  year={2023},
  publisher={Elsevier}
}

@inproceedings{sebastian2022influence,
  title={Influence of crossflow Mach number on spanwise-inclined jet injection},
  author={Sebastian, Robin and Schreyer, Anne-Marie},
  booktitle={AIAA Scitech 2022 Forum},
  pages={1363},
  year={2022}
}

@article{qi2023large,
  title={Large-eddy simulation of a hypersonic turbulent boundary layer over a compression corner},
  author={Qi, Han and Li, Xinliang and Ji, Xiangxin and Tong, Fulin and Yu, Changping},
  journal={AIP Advances},
  volume={13},
  number={2},
  year={2023},
  publisher={AIP Publishing}
}

@article{guo2024wall,
  title={Wall skin friction analysis in a hypersonic turbulent boundary layer over a compression ramp},
  author={Guo, Tongbiao and Zhang, Ji and Zhu, Yanhua and Li, Xinliang},
  journal={Journal of Fluid Mechanics},
  volume={988},
  pages={A23},
  year={2024},
  publisher={Cambridge University Press}
}

@article{di2024stagnation,
  title={Stagnation enthalpy effects on hypersonic turbulent compression corner flow at moderate Reynolds numbers},
  author={Di Renzo, M and Williams, CT and Pirozzoli, S},
  journal={Physical Review Fluids},
  volume={9},
  number={3},
  pages={033401},
  year={2024},
  publisher={APS}
}

@inproceedings{bhagwandin2021shock,
  title={LES of Shock-Turbulent Boundary Layer Interaction over a Mach 10 Hollow Cylinder with Flare.},
  author={Bhagwandin, Vishal A and Martin, Pino},
  booktitle={AIAA AVIATION 2021 FORUM},
  pages={2820},
  year={2021}
}

@article{ninni2023simulation,
  title={Simulation of High-Enthalpy Turbulent Shock Wave/Boundary Layer Interaction Using a RANS Approach},
  author={Ninni, Davide and Bonelli, Francesco and Pascazio, Giuseppe},
  journal={Aerotecnica Missili \& Spazio},
  volume={102},
  number={4},
  pages={323--335},
  year={2023},
  publisher={Springer}
}

@article{helm2021scaling,
  title={Scaling of hypersonic shock/turbulent boundary layer interactions},
  author={Helm, Clara M and Mart{\'\i}n, MP},
  journal={Physical Review Fluids},
  volume={6},
  number={7},
  pages={074607},
  year={2021},
  publisher={APS}
}

@article{helm2021characterization,
  title={Characterization of the shear layer in separated shock/turbulent boundary layer interactions},
  author={Helm, Clara M and Mart{\'\i}n, M Pino and Williams, Owen JH},
  journal={Journal of Fluid Mechanics},
  volume={912},
  pages={A7},
  year={2021},
  publisher={Cambridge University Press}
}

@inproceedings{muir2024assessment,
  title={Assessment of Reynolds-Averaged Navier-Stokes Simulations for Predicting Scaling Trends in Shock-Separated Boundary Layers},
  author={Muir, David P and Martin, Pino},
  booktitle={AIAA AVIATION FORUM AND ASCEND 2024},
  pages={3550},
  year={2024}
}

@inproceedings{bhagwandin2023wall,
  title={Wall-Resolved LES of Mach 6 BoLT-2 Hypersonic Vehicle},
  author={Bhagwandin, Vishal A and Martin, Pino},
  booktitle={AIAA AVIATION 2023 Forum},
  pages={3848},
  year={2023}
}

@article{grube2021reynolds,
  title={Reynolds stress anisotropy in shock/isotropic turbulence interactions},
  author={Grube, Nathan E and Mart{\'\i}n, M Pino},
  journal={Journal of Fluid Mechanics},
  volume={913},
  pages={A19},
  year={2021},
  publisher={Cambridge University Press}
}

@article{huete2021thermochemical,
  title={Thermochemical effects on hypersonic shock waves interacting with weak turbulence},
  author={Huete, C and Cuadra, A and Vera, M and Urzay, J},
  journal={Physics of Fluids},
  volume={33},
  number={8},
  year={2021},
  publisher={AIP Publishing}
}

@inproceedings{bhagwandin2019shock,
  title={Shock-Turbulent Boundary Layer Interactions in Separated Compression Corners at Mach 10.},
  author={Bhagwandin, Vishal A and Helm, Clara M and Martin, Pino},
  booktitle={AIAA Scitech 2019 Forum},
  pages={1129},
  year={2019}
}

@misc{yuting2021scaling,
  title={Scaling of interaction lengths for hypersonic shock wave/turbulent boundary layer interactions},
  author={Yuting, HONG and Zhufei, LI and Jiming, YANG},
  journal={Chinese Journal of Aeronautics},
  volume={34},
  number={5},
  pages={504--509},
  year={2021},
  publisher={Elsevier}
}

@article{rathi2024simulation,
  title={Simulation of Hypersonic Shock-Boundary Layer Interaction Using Shock-Strength Dependent Turbulence Model},
  author={Rathi, Harsha and Sinha, Krishnendu},
  journal={AIAA Journal},
  pages={1--14},
  year={2024},
  publisher={American Institute of Aeronautics and Astronautics}
}

@inproceedings{brooks2017mach,
  title={Mach 10 PIV flow field measurements of a turbulent boundary layer and shock turbulent boundary layer interaction},
  author={Brooks, Jonathan and Gupta, Ashwani and Marineau, Eric C and Smith, Michael},
  booktitle={33rd AIAA aerodynamic measurement technology and ground testing conference},
  pages={3325},
  year={2017}
}

@inproceedings{helm2016new,
  title={New LES of a hypersonic shock/turbulent boundary layer interaction},
  author={Helm, Clara M and Martin, M Pino},
  booktitle={54th AIAA Aerospace Sciences Meeting},
  pages={0346},
  year={2016}
}

@article{whalen2020hypersonic,
  title={Hypersonic fluid--structure interactions in compression corner shock-wave/boundary-layer interaction},
  author={Whalen, Thomas J and Sch{\"o}neich, Antonio Giovanni and Laurence, Stuart J and Sullivan, Bryson T and Bodony, Daniel J and Freydin, Maxim and Dowell, Earl H and Buck, Gregory M},
  journal={AIAA journal},
  volume={58},
  number={9},
  pages={4090--4105},
  year={2020},
  publisher={American Institute of Aeronautics and Astronautics}
}

@inproceedings{whalen2019unsteady,
  title={Unsteady surface and flowfield measurements in ramp-induced turbulent and transitional shock-wave boundary-layer interactions at Mach 6},
  author={Whalen, Thomas J and Kennedy, Richard E and Laurence, Stuart J and Sullivan, Bryson and Bodony, Daniel J and Buck, Gregory},
  booktitle={AIAA Scitech 2019 Forum},
  pages={1127},
  year={2019}
}

@article{martin2007direct,
  title={Direct numerical simulation of hypersonic turbulent boundary layers. Part 1. Initialization and comparison with experiments},
  author={Martin, M Pino},
  journal={Journal of Fluid Mechanics},
  volume={570},
  pages={347--364},
  year={2007},
  publisher={Cambridge University Press}
}

@inproceedings{bookey2005new,
  title={New experimental data of STBLI at DNS/LES accessible Reynolds numbers},
  author={Bookey, Patrick and Wyckham, Christopher and Smits, Alexander and Martin, Pino},
  booktitle={43rd AIAA Aerospace Sciences Meeting and Exhibit},
  pages={309},
  year={2005}
}

@article{duan2016pressure,
  title={Pressure fluctuations induced by a hypersonic turbulent boundary layer},
  author={Duan, Lian and Choudhari, Meelan M and Zhang, Chao},
  journal={Journal of Fluid Mechanics},
  volume={804},
  pages={578--607},
  year={2016},
  publisher={Cambridge University Press}
}

@article{martin1998effect,
  title={Effect of chemical reactions on decaying isotropic turbulence},
  author={Mart{\i}n, M Pino and Candler, Graham V},
  journal={Physics of Fluids},
  volume={10},
  number={7},
  pages={1715--1724},
  year={1998},
  publisher={American Institute of Physics}
}

@article{duan2011assessment,
  title={Assessment of turbulence-chemistry interaction in hypersonic turbulent boundary layers},
  author={Duan, Lian and Mart{\'\i}n, M Pino},
  journal={AIAA journal},
  volume={49},
  number={1},
  pages={172--184},
  year={2011}
}

@article{reynolds1895iv,
  title={IV. On the dynamical theory of incompressible viscous fluids and the determination of the criterion},
  author={Reynolds, Osborne},
  journal={Philosophical transactions of the royal society of london.(a.)},
  number={186},
  pages={123--164},
  year={1895},
  publisher={The Royal Society London}
}

@article{favre1965equations,
  title={Equations des gaz turbulents compressibles},
  author={Favre, A},
  journal={J. de Mecanique},
  volume={4},
  number={3},
  pages={361},
  year={1965}
}


@book{prandtl1945neues,
  title={{\"U}ber ein neues Formelsystem f{\"u}r die ausgebildete Turbulenz},
  author={Prandtl, Ludwig},
  year={1945},
  publisher={Vandenhoeck \& Ruprecht}
}


@article{zhang2022review,
  title={A review of the mathematical modeling of equilibrium and nonequilibrium hypersonic flows},
  author={Zhang, Wenqing and Zhang, Zhijun and Wang, Xiaowei and Su, Tianyi},
  journal={Advances in Aerodynamics},
  volume={4},
  number={1},
  pages={38},
  year={2022},
  publisher={Springer}
}

@article{guohua2012assessment,
  title={Assessment of two turbulence models and some compressibility corrections for hypersonic compression corners by high-order difference schemes},
  author={Guohua, TU and Xiaogang, DENG and Meiliang, MAO},
  journal={Chinese Journal of Aeronautics},
  volume={25},
  number={1},
  pages={25--32},
  year={2012},
  publisher={Elsevier}
}

@article{zhu2020analysis,
  title={Analysis of compressibility corrections for turbulence models in hypersonic boundary-layer applications},
  author={Zhu, Zhibin and Zhang, Xuejun and Wang, Xun and Zhang, Liang},
  journal={Journal of Spacecraft and Rockets},
  volume={57},
  number={2},
  pages={364--372},
  year={2020},
  publisher={American Institute of Aeronautics and Astronautics}
}

@article{barone2022internal,
  title={Internal energy balance and aerodynamic heating predictions for hypersonic turbulent boundary layers},
  author={Barone, Matthew and Nicholson, Gary L and Duan, Lian},
  journal={Physical Review Fluids},
  volume={7},
  number={8},
  pages={084604},
  year={2022},
  publisher={APS}
}

@article{marchenay2022hypersonic,
  title={Hypersonic Turbulent Flow Reynolds-Averaged Navier--Stokes Simulations with Roughness and Blowing Effects},
  author={Marchenay, Yann and Olazabal Loum{\'e}, M and Chedevergne, Fran{\c{c}}ois},
  journal={Journal of Spacecraft and Rockets},
  volume={59},
  number={5},
  pages={1686--1696},
  year={2022},
  publisher={American Institute of Aeronautics and Astronautics}
}

@inproceedings{buck2021rans,
  title={On RANS turbulence models for high-speed applications},
  author={Buck, Axel and Mundt, Christian},
  booktitle={AIAA Scitech 2021 Forum},
  pages={1744},
  year={2021}
}

@inproceedings{oliver2007assessment,
  title={Assessment of turbulent shock-boundary layer interaction computations using the OVERFLOW code},
  author={Oliver, Anthony and Lillard, Randolph and Schwing, Alan and Blaisdell, Gregory and Lyrintzis, Anastasios},
  booktitle={45th AIAA Aerospace Sciences Meeting and Exhibit},
  pages={104},
  year={2007}
}

@inproceedings{huang2017high,
  title={High-Mach-number turbulence modeling using machine learning and direct numerical simulation database},
  author={Huang, Junji and Duan, Lian and Wang, Jianxun and Sun, Rui and Xiao, Heng},
  booktitle={55th AIAA Aerospace Sciences Meeting},
  pages={0315},
  year={2017}
}

@article{wang2019prediction,
  title={{Prediction of Reynolds stresses in high-Mach-number turbulent boundary layers using physics-informed machine learning}},
  author={Wang, Jian-Xun and Huang, Junji and Duan, Lian and Xiao, Heng},
  journal={Theoretical and Computational Fluid Dynamics},
  volume={33},
  pages={1--19},
  year={2019},
  publisher={Springer}
}

@article{chowdhary2022calibrating,
  title={Calibrating hypersonic turbulence flow models with the HIFiRE-1 experiment using data-driven machine-learned models},
  author={Chowdhary, Kenny and Hoang, Chi and Lee, Kookjin and Ray, Jaideep and Weirs, V Gregory and Carnes, Brian},
  journal={Computer Methods in Applied Mechanics and Engineering},
  volume={401},
  pages={115396},
  year={2022},
  publisher={Elsevier}
}

@article{cherroud2023space,
  title={Space-dependent Aggregation of Stochastic Data-driven Turbulence Models},
  author={Cherroud, S. and Merle, X. and Cinnella, P. and Gloerfelt, X.},
  journal={arXiv preprint arXiv:2306.16996},
  year={2023}
}

@article{oulghelou2024machine,
  title={Machine-learning-assisted Blending of Data-Driven Turbulence Models},
  author={Oulghelou, M. and Cherroud, S. and Merle, X. and Cinnella, P.},
  journal={arXiv preprint arXiv:2410.14431},
  year={2024}
}

@article{rincon2023progressive,
  title={Progressive augmentation of Reynolds stress tensor models for secondary flow prediction by computational fluid dynamics driven surrogate optimisation},
  author={Rinc{\'o}n, Mario Javier and Amarloo, Ali and Reclari, Martino and Yang, Xiang IA and Abkar, Mahdi},
  journal={International Journal of Heat and Fluid Flow},
  volume={104},
  pages={109242},
  year={2023},
  publisher={Elsevier}
}

@article{fang2023toward,
  title={Toward more general turbulence models via multicase computational-fluid-dynamics-driven training},
  author={Fang, Yuan and Zhao, Yaomin and Waschkowski, Fabian and Ooi, Andrew SH and Sandberg, Richard D},
  journal={AIAA Journal},
  volume={61},
  number={5},
  pages={2100--2115},
  year={2023},
  publisher={American Institute of Aeronautics and Astronautics}
}

@article{huang2022direct,
  title={Direct numerical simulation of hypersonic turbulent boundary layers: effect of spatial evolution and Reynolds number},
  author={Huang, Junji and Duan, Lian and Choudhari, Meelan M},
  journal={Journal of Fluid Mechanics},
  volume={937},
  pages={A3},
  year={2022},
  publisher={Cambridge University Press}
}

@inproceedings{dann2007cfd,
  title={CFD designed experiments for shock wave/boundary layer interactions in hypersonic ducted flows},
  author={Dann, AG and Morgan, RG},
  booktitle={Proceedings of the 16th Australasian Fluid Mechanics Conference, 16AFMC},
  volume={1},
  pages={1304--1308},
  year={2007},
  organization={Citeseer}
}

@techreport{dilley2001evaluation,
  title={Evaluation of CFD turbulent heating prediction techniques and comparison with hypersonic experimental data},
  author={Dilley, Arthur D and McClinton, Charles R},
  year={2001}
}

@article{hejranfar2012dual,
  title={Dual-code solution procedure for efficient computing equilibrium hypersonic axisymmetric transitional/turbulent flows},
  author={Hejranfar, Kazem and Esfahanian, Vahid and Kamali-Moghadam, Ramin},
  journal={Aerospace Science and Technology},
  volume={21},
  number={1},
  pages={64--74},
  year={2012},
  publisher={Elsevier}
}

@inproceedings{horstman1987prediction,
  title={Prediction of hypersonic shock-wave/turbulent-boundary-layer interaction flows},
  author={Horstman, CC},
  booktitle={19th AIAA, Fluid Dynamics, Plasma Dynamics, and Lasers Conference},
  pages={1367},
  year={1987}
}

@inproceedings{kim1988hypersonic,
  title={Hypersonic turbulent wall boundary layer computations},
  author={KIM, S and HARLOFF, G},
  booktitle={24th Joint Propulsion Conference},
  pages={2829},
  year={1988}
}

@inproceedings{narayanswami1993numerical,
  title={Numerical simulation of crossing/turbulent boundary layer interaction at Mach 8.3 comparison of zero and two-equation turbulence models},
  author={Narayanswami, N and HORSTMAN, C and KNIGHT, D},
  booktitle={31st Aerospace Sciences Meeting},
  pages={779},
  year={1993}
}

@inproceedings{ozgun2015hypersonic,
  title={Hypersonic Flow Analysis of Re-entry Vehicles Using Three Dimensional Navier-Stokes Equations},
  author={Ozgun, Muharrem and Eyi, Sinan},
  booktitle={13th International Energy Conversion Engineering Conference},
  pages={3881},
  year={2015}
}

@article{panaras2015turbulence,
  title={Turbulence modeling of flows with extensive crossflow separation},
  author={Panaras, Argyris G},
  journal={Aerospace},
  volume={2},
  number={3},
  pages={461--481},
  year={2015},
  publisher={MDPI}
}

@article{sarkar1992pressure,
  title={The pressure--dilatation correlation in compressible flows},
  author={Sarkar, S},
  journal={Physics of Fluids A: Fluid Dynamics},
  volume={4},
  number={12},
  pages={2674--2682},
  year={1992},
  publisher={American Institute of Physics}
}

@article{so1998morkovin,
  title={Morkovin hypothesis and the modeling of wall-bounded compressible turbulent flows},
  author={So, RMC and Gatski, TB and Sommer, TP},
  journal={AIAA journal},
  volume={36},
  number={9},
  pages={1583--1592},
  year={1998}
}


@article{sinha2003modeling,
  title={Modeling shock unsteadiness in shock/turbulence interaction},
  author={Sinha, Krishnendu and Mahesh, Krishnan and Candler, Graham V},
  journal={Physics of fluids},
  volume={15},
  number={8},
  pages={2290--2297},
  year={2003},
  publisher={American Institute of Physics}
}

@article{veera2009modeling,
  title={Modeling the effect of upstream temperature fluctuations on shock/homogeneous turbulence interaction},
  author={Veera, Vijay K and Sinha, Krishnendu},
  journal={Physics of fluids},
  volume={21},
  number={2},
  year={2009},
  publisher={AIP Publishing}
}

@article{marchenay2022hypersonic,
  title={Hypersonic Turbulent Flow Reynolds-Averaged Navier--Stokes Simulations with Roughness and Blowing Effects},
  author={Marchenay, Yann and Olazabal Loum{\'e}, M and Chedevergne, Fran{\c{c}}ois},
  journal={Journal of Spacecraft and Rockets},
  volume={59},
  number={5},
  pages={1686--1696},
  year={2022},
  publisher={American Institute of Aeronautics and Astronautics}
}

@article{nicholson2024direct,
  title={Direct Numerical Simulation Database of High-Speed Flow over Parameterized Curved Walls},
  author={Nicholson, Gary L and Duan, Lian and Bisek, Nicholas J},
  journal={AIAA Journal},
  volume={62},
  number={6},
  pages={2095--2118},
  year={2024},
  publisher={American Institute of Aeronautics and Astronautics}
}

@article{marvin1983turbulence,
  title={Turbulence modeling for computational aerodynamics},
  author={Marvin, Joseph G},
  journal={AIAA Journal},
  volume={21},
  number={7},
  pages={941--955},
  year={1983}
}

@inproceedings{bardina1994three,
  title={Three-dimensional Navier-Stokes method with two-equation turbulence models for efficient numerical simulation of hypersonic flows},
  author={Bardina, J},
  booktitle={30th Joint Propulsion Conference and Exhibit},
  pages={2950},
  year={1994}
}


@techreport{settles1991,
  title={Hypersonic shock/boundary-layer interaction database},
  author={Settles, GS and Dodson, LJ},
  year={1991},
  institution={NASA CR 177577}
}

@article{bose2018wall,
  title={Wall-modeled large-eddy simulation for complex turbulent flows},
  author={Bose, Sanjeeb T and Park, George Ilhwan},
  journal={Annual review of fluid mechanics},
  volume={50},
  number={1},
  pages={535--561},
  year={2018},
  publisher={Annual Reviews}
}

@article{mettu2022wall,
  title={Wall-modeled large eddy simulation of high speed flows},
  author={Mettu, Balachandra R and Subbareddy, Pramod K},
  journal={AIAA journal},
  volume={60},
  number={7},
  pages={4302--4324},
  year={2022},
  publisher={American Institute of Aeronautics and Astronautics}
}

@inproceedings{zangeneh2021wall,
  title={Wall-modeled large-eddy simulation of hypersonic turbulent boundary-layers},
  author={Zangeneh, Rozie},
  booktitle={AIAA Scitech 2021 Forum},
  pages={1076},
  year={2021}
}
 @article{Schwarzkopf_Livescu_Baltzer_Gore_Ristorcelli_2016, title={A Two-length Scale Turbulence Model for Single-phase Multi-fluid Mixing}, abstractNote={A two-length scale, second moment turbulence model (Reynolds averaged Navier-Stokes, RANS) is proposed to capture a wide variety of single-phase flows, spanning from incompressible flows with single fluids and mixtures of different density fluids (variable density flows) to flows over shock waves. The two-length scale model was developed to address an inconsistency present in the single-length scale models, e.g. the inability to match both variable density homogeneous Rayleigh-Taylor turbulence and Rayleigh-Taylor induced turbulence, as well as the inability to match both homogeneous shear and free shear flows. The two-length scale model focuses on separating the decay and transport length scales, as the two physical processes are generally different in inhomogeneous turbulence. This allows reasonable comparisons with statistics and spreading rates over such a wide range of turbulent flows using a common set of model coefficients. The specific canonical flows considered for calibrating the model include homogeneous shear, single-phase incompressible shear driven turbulence, variable density homogeneous Rayleigh-Taylor turbulence, Rayleigh-Taylor induced turbulence, and shocked isotropic turbulence. The second moment model shows to compare reasonably well with direct numerical simulations (DNS), experiments, and theory in most cases. The model was then applied to variable density shear layer and shock tube data and shows to be in reasonable agreement with DNS and experiments. The importance of using DNS to calibrate and assess RANS type turbulence models is also highlighted.}, author={Schwarzkopf, J D and Livescu, D and Baltzer, J R and Gore, R A and Ristorcelli, J R}, year={2016}, language={en} }


 @inbook{Karl_Hickey_Lacombe_2019, address={Cham}, title={Reynolds Stress Models for Shock-Turbulence Interaction}, ISBN={978-3-319-91019-2}, url={http://link.springer.com/10.1007/978-3-319-91020-8_60}, DOI={10.1007/978-3-319-91020-8_60}, abstractNote={A systematic deﬁciency of current turbulence models which are based on the Reynolds-averaged Navier-Stokes equations (RANS) is their inability to correctly predict the interaction of turbulence with shocks. This is because RANS models do not account for the unsteady motion or fragmentation of the shock wave within the interaction zone. Typically, signiﬁcant over-prediction of the turbulent energy ampliﬁcation occurs without dedicated adjustment of the applied turbulence model.}, booktitle={31st International Symposium on Shock Waves 1}, publisher={Springer International Publishing}, author={Karl, Sebastian and Hickey, Jean-Pierre and Lacombe, Francis}, editor={Sasoh, Akihiro and Aoki, Toshiyuki and Katayama, Masahide}, year={2019}, pages={511–517}, language={en} }

@article{spalart2009detached,
  title={Detached-eddy simulation},
  author={Spalart, Philippe R},
  journal={Annual review of fluid mechanics},
  volume={41},
  number={1},
  pages={181--202},
  year={2009},
  publisher={Annual Reviews}
}

@article{moin1998direct,
  title={Direct numerical simulation: a tool in turbulence research},
  author={Moin, Parviz and Mahesh, Krishnan},
  journal={Annual review of fluid mechanics},
  volume={30},
  number={1},
  pages={539--578},
  year={1998},
  publisher={Annual Reviews 4139 El Camino Way, PO Box 10139, Palo Alto, CA 94303-0139, USA}
}

@article{zhiyin2015large,
  title={Large-eddy simulation: Past, present and the future},
  author={Zhiyin, Yang},
  journal={Chinese journal of Aeronautics},
  volume={28},
  number={1},
  pages={11--24},
  year={2015},
  publisher={Elsevier}
}

@article{horstman1972turbulent,
  title={Turbulent properties of a compressible boundary layer.},
  author={Horstman, CC and Owen, FK},
  journal={AIAA Journal},
  volume={10},
  number={11},
  pages={1418--1424},
  year={1972}
}

@article{owen1972structure,
  title={On the structure of hypersonic turbulent boundary layers},
  author={Owen, FK and Horstman, CC},
  journal={Journal of Fluid Mechanics},
  volume={53},
  number={4},
  pages={611--636},
  year={1972},
  publisher={Cambridge University Press}
}

@article{owen1975mean,
  title={Mean and fluctuating flow measurements of a fully-developed, non-adiabatic, hypersonic boundary layer},
  author={Owen, FK and Horstman, CC and Kussoy, MI},
  journal={Journal of Fluid Mechanics},
  volume={70},
  number={2},
  pages={393--413},
  year={1975},
  publisher={Cambridge University Press}
}




@article{PaChJo24,
	abstract = { We develop a neural-network-based variable turbulent Prandtl number model for the k-eps turbulence model for improved wall heating predictions in hypersonic shock--boundary-layer interactions (SBLIs). The model is developed by performing a finite-dimensional field inference for a spatially varying turbulent Prandtl number on six canonical SBLIs: three compression ramps at Mach 8 and three impinging shocks at Mach 5. The inference results identify a turbulent Prandtl number that reduces wall heating by systematically directing heat transfer away from the wall. An ensemble of Lipschitz-continuous neural networks is then trained on the inferred turbulent Prandtl number fields to develop a predictive model. We evaluate the resulting variable turbulent Prandtl number model on a suite of test cases, including the hollow cylinder flare and HIFiRE ground test experiments. The machine-learning-augmented model systematically increases Prt near the wall to reduce negative turbulent heat flux while decreasing Prt away from the wall to enhance positive turbulent heat flux, collectively reducing overall heat transfer to the surface. Results show that the learned model consistently improves peak heating predictions by 40--70\% compared to the baseline k--ϵ model, a k--ϵ model augmented with various high-speed corrections, and the shear stress transport model across a range of conditions. },
	author = {Parish, Eric and Ching, David S. and Jordan, Cyrus and Nicholson, Gary and Miller, Nathan E. and Beresh, Steven and Barone, Matthew and Gupta, Niloy and Duraisamy, Karthik},
	doi = {10.2514/1.J064745},
	eprint = {https://doi.org/10.2514/1.J064745},
	journal = {AIAA Journal},
	number = {0},
	pages = {1-22},
	title = {Data-Driven Turbulent Prandtl Number Modeling for Hypersonic Shock--Boundary-Layer Interactions},
	url = {https://doi.org/10.2514/1.J064745},
	volume = {0},
	year = {0},
	bdsk-url-1 = {https://doi.org/10.2514/1.J064745}}

@article{mikulla1976turbulence,
  title={Turbulence measurements in hypersonic shock-wave boundary-layer interaction flows},
  author={Mikulla, Vo and Horstman, Co C},
  journal={AIAA Journal},
  volume={14},
  number={5},
  pages={568--575},
  year={1976}
}

@inproceedings{sahoo2009effects,
  title={Effects of roughness on a turbulent bloundary layer in hypersonic flow},
  author={Sahoo, Dipankar and Schultze, Marco and Smits, Alexander},
  booktitle={39th AIAA Fluid Dynamics Conference},
  pages={3678},
  year={2009}
}

@book{baumgartner1997turbulence,
  title={Turbulence structure in a hypersonic boundary layer},
  author={Baumgartner, Mark Lawrence},
  year={1997},
  publisher={Princeton University}
}

@inproceedings{mcginley1994turbulence,
  title={Turbulence measurements in a Mach 11 helium boundary layer},
  author={McGinley, C and Spina, E and Sheplak, M},
  booktitle={Fluid Dynamics Conference},
  pages={2364},
  year={1994}
}

@inproceedings{nance1999turbulence,
  title={Turbulence modeling of shock-dominated flows with a k-zeta formulation},
  author={Nance, Robert and Hassan, H},
  booktitle={37th Aerospace Sciences Meeting and Exhibit},
  pages={153},
  year={1999}
}

@article{robinson1998further,
  title={Further Development of the k-?(Enstrophy) Turbulence Closure Model},
  author={Robinson, DF and Hassan, HA},
  journal={AIAA journal},
  volume={36},
  number={10},
  pages={1825--1833},
  year={1998}
}

@inproceedings{smith1995prediction,
  title={Prediction of hypersonic shock wave turbulent boundary layer interactions with the kl two equation turbulence model},
  author={Smith, Brian},
  booktitle={33rd Aerospace Sciences Meeting and Exhibit},
  pages={232},
  year={1995}
}

@inproceedings{coakley1983turbulence,
  title={Turbulence modeling methods for the compressible Navier-Stokes equations},
  author={Coakley, Ti},
  booktitle={16th fluid and plasmadynamics conference},
  pages={1693},
  year={1983}
}

@article{leschziner2006modelling,
  title={Modelling turbulent separated flow in the context of aerodynamic applications},
  author={Leschziner, MA},
  journal={Fluid dynamics research},
  volume={38},
  number={2-3},
  pages={174--210},
  year={2006},
  publisher={Elsevier}
}

@article{shih1993realisable,
  title={A Realisable Reynolds Stress Algebraic Equation Model},
  author={SHIH, TH},
  journal={NASA TM-105993},
  year={1993}
}

@inproceedings{lien1996low,
  title={Low-Reynolds-number eddy-viscosity modelling based on non-linear stress-strain/vorticity relations},
  author={Lien, Fue-Sang},
  booktitle={Proc. 3rd Symposium On Engineering Turbulence Modelling and Measurements},
  pages={1--10},
  year={1996}
}

@article{coleman1972heat,
  title={Heat transfer from hypersonic turbulent flow at a wedge compression corner},
  author={Coleman, GT and Stollery, JL},
  journal={Journal of Fluid Mechanics},
  volume={56},
  number={4},
  pages={741--752},
  year={1972},
  publisher={Cambridge University Press}
}

@article{holden1992turbulent,
  title={Turbulent boundary layer development on curved compression surfaces},
  author={Holden, MS},
  journal={Calspan Report No},
  pages={7724--1},
  year={1992}
}

@article{craft2000progress,
  title={Progress in the use of non-linear two-equation models in the computation of convective heat-transfer in impinging and separated flows},
  author={Craft, TJ and Iacovides, H and Yoon, JH},
  journal={Flow, Turbulence and Combustion},
  volume={63},
  pages={59--80},
  year={2000},
  publisher={Springer}
}

@article{craft1996development,
  title={Development and application of a cubic eddy-viscosity model of turbulence},
  author={Craft, TJ and Launder, BE and Suga, K},
  journal={International Journal of Heat and Fluid Flow},
  volume={17},
  number={2},
  pages={108--115},
  year={1996},
  publisher={Elsevier}
}


@incollection{rung1999assessment,
  title={Assessment of explicit algebraic stress models in transonic flows},
  author={Rung, Thomas and L{\"u}bcke, H and Franke, M and Xue, L and Thiele, Frank and Fu, Song},
  booktitle={Engineering Turbulence Modelling and Experiments 4},
  pages={659--668},
  year={1999},
  publisher={Elsevier}
}

@article{gatski1993explicit,
  title={On explicit algebraic stress models for complex turbulent flows},
  author={Gatski, Thomas B and Speziale, Charles G},
  journal={Journal of fluid Mechanics},
  volume={254},
  pages={59--78},
  year={1993},
  publisher={Cambridge University Press}
}

@article{speziale1991modelling,
  title={Modelling the pressure--strain correlation of turbulence: an invariant dynamical systems approach},
  author={Speziale, Charles G and Sarkar, Sutanu and Gatski, Thomas B},
  journal={Journal of fluid mechanics},
  volume={227},
  pages={245--272},
  year={1991},
  publisher={Cambridge University Press}
}

@misc{M5DNS_SBLI,
    title = {NASA TMR},
    howpublished =  {\url{https://turbmodels.larc.nasa.gov/Other_DNS_Data/highspeed_curvedwalls.html}},
    author = {Nicholson, et al.},
    year = {2024},
    note = {Last accessed on Oct --, 2024}
}

@article{prince2005experiments,
  title={Experiments on the hypersonic turbulent shock-wave/boundary-layer interaction and the effects of surface roughness},
  author={Prince, SA and Vannahme, M and Stollery, JL},
  journal={The Aeronautical Journal},
  volume={109},
  number={1094},
  pages={177--184},
  year={2005},
  publisher={Cambridge University Press}
}

@article{WaMaHo08,
  author = "T. Wadhams and M. MacLean and M. Holden and E. Mundy",
  title = "Ground test studies of the {HIFiRE-1} transition experiment {Part 1: Experimental} results",
  journal = "J. Spacecraft Rockets",
  volume = "45",
  number = 6,
  year = 2008,
  pages = "1134--1148",
  doi = "doi: 10.2514/138338",
}


@inproceedings{holden2008review,
  title={A review of experimental studies of surface roughness and blowing on the heat transfer and skin friction to nosetips and slender cones in high mach numbers flows},
  author={Holden, Michael and Wadhams, Timothy and Mundy, Erik},
  booktitle={40th Thermophysics Conference},
  pages={3907},
  year={2008}
}


@inproceedings{sahoo2009effects,
  title={Effects of roughness on a turbulent bloundary layer in hypersonic flow},
  author={Sahoo, Dipankar and Schultze, Marco and Smits, Alexander},
  booktitle={39th AIAA Fluid Dynamics Conference},
  pages={3678},
  year={2009}
}

@article{peltier2016crosshatch,
  title={Crosshatch roughness distortions on a hypersonic turbulent boundary layer},
  author={Peltier, SJ and Humble, RA and Bowersox, RDW},
  journal={Physics of Fluids},
  volume={28},
  number={4},
  year={2016},
  publisher={AIP Publishing}
}

@book{berg1977surface,
  title={SURFACE ROUGHNESS EFFECTS ON THE HYPERSONIC TURBULENT BOUNDARY LAYER.},
  author={Berg, Dale Evan},
  year={1977},
  publisher={California Institute of Technology}
}

@inproceedings{finson1980effect,
  title={The effect of surface roughness character on turbulent re-entry heating},
  author={Finson, M and Clarke, A},
  booktitle={15th Thermophysics Conference},
  pages={1459},
  year={1980}
}


@article{aupoix2015roughness,
  title={Roughness corrections for the k--$\omega$ shear stress transport model: Status and proposals},
  author={Aupoix, B},
  journal={Journal of Fluids Engineering},
  volume={137},
  number={2},
  pages={021202},
  year={2015},
  publisher={American Society of Mechanical Engineers}
}

@article{aupoix2015improved,
  title={Improved heat transfer predictions on rough surfaces},
  author={Aupoix, B},
  journal={International Journal of Heat and Fluid Flow},
  volume={56},
  pages={160--171},
  year={2015},
  publisher={Elsevier}
}

@article{marchenay2021modeling,
  title={Modeling of combined effects of surface roughness and blowing for Reynolds-averaged Navier--Stokes turbulence models},
  author={Marchenay, Yann and Chedevergne, Fran{\c{c}}ois and Olazabal Loum{\'e}, M},
  journal={Physics of Fluids},
  volume={33},
  number={4},
  year={2021},
  publisher={AIP Publishing}
}

@inproceedings{olazabal2017study,
  title={Study on k-$\omega$ shear stress transport model corrections applied to rough wall turbulent hypersonic boundary layers},
  author={Olazabal-Loum{\'e}, M and Danvin, Florian and Mathiaud, Julien and Aupoix, Bertrand and Toulouse, ONERA},
  booktitle={Seventh European Conference for Aeronautics and Space Sciences},
  year={2017}
}

@inproceedings{olazabal2019roughness,
  title={Roughness corrections applied to the simulation of turbulent hypersonic flows},
  author={Olazabal-Loum{\'e}, Marina and Chedevergne, Fran{\c{c}}ois and Danvin, Florian and Mathiaud, Julien},
  booktitle={EUCASS 2019},
  year={2019}
}

@article{wilcox1988reassessment,
  title={Reassessment of the scale-determining equation for advanced turbulence models},
  author={Wilcox, David C},
  journal={AIAA journal},
  volume={26},
  number={11},
  pages={1299--1310},
  year={1988}
}

@article{goddard1959effect,
  title={Effect of uniformly distributed roughness on turbulent skin-friction drag at supersonic speeds},
  author={Goddard Jr, Frank E},
  journal={Journal of the Aerospace Sciences},
  volume={26},
  number={1},
  pages={1--15},
  year={1959}
}

@article{lin1982turbulence,
  title={Turbulence models for high-speed, rough-wall boundary layers},
  author={Lin, TC and Bywater, RJ},
  journal={AIAA Journal},
  volume={20},
  number={3},
  pages={325--333},
  year={1982}
}

@article{choi2012grid,
  title={Grid-point requirements for large eddy simulation: Chapman’s estimates revisited},
  author={Choi, Haecheon and Moin, Parviz},
  journal={Physics of fluids},
  volume={24},
  number={1},
  year={2012},
  publisher={AIP Publishing}
}

@article{yang2021grid,
  title={Grid-point and time-step requirements for direct numerical simulation and large-eddy simulation},
  author={Yang, Xiang IA and Griffin, Kevin P},
  journal={Physics of Fluids},
  volume={33},
  number={1},
  year={2021},
  publisher={AIP Publishing}
}


@article{goyne2003skin,
  title={Skin-friction measurements in high-enthalpy hypersonic boundary layers},
  author={Goyne, CP and Stalker, RJ and Paull, A},
  journal={Journal of Fluid Mechanics},
  volume={485},
  pages={1--32},
  year={2003},
  publisher={Cambridge University Press}
}

@inproceedings{fang2015large,
  title={Large-eddy simulation of a three-dimensional hypersonic shock wave turbulent boundary layer interaction of a single-fin},
  author={Fang, Jian and Yao, Yufeng and Zheltovodov, Alexander and Lu, Lipeng},
  booktitle={53rd AIAA Aerospace Sciences Meeting},
  pages={1062},
  year={2015}
}


@article{fang2017investigation,
  title={Investigation of three-dimensional shock wave/turbulent-boundary-layer interaction initiated by a single fin},
  author={Fang, Jian and Yao, Yufeng and Zheltovodov, Alexandr A and Lu, Lipeng},
  journal={AIAA Journal},
  volume={55},
  number={2},
  pages={509--523},
  year={2017},
  publisher={American Institute of Aeronautics and Astronautics}
}

@inproceedings{kianvashrad2021large,
  title={Large Eddy Simulation of Hypersonic Cold Wall Flat Plate},
  author={Kianvashrad, Nadia and Knight, Doyle D},
  booktitle={AIAA AVIATION 2021 FORUM},
  pages={2882},
  year={2021}
}

@inproceedings{knight2024large,
  title={Large Eddy Simulation of Cold Wall Hypersonic Turbulent Boundary Layers},
  author={Knight, Doyle D},
  booktitle={AIAA AVIATION FORUM AND ASCEND 2024},
  pages={3966},
  year={2024}
}

@inproceedings{spalart1992one,
  title={A one-equation turbulence model for aerodynamic flows},
  author={Spalart, Philippe and Allmaras, Steven},
  booktitle={30th aerospace sciences meeting and exhibit},
  pages={439},
  year={1992}
}

@book{smith1967numerical,
  title={Numerical solution of the turbulent-boundary-layer equations},
  author={Smith, AMOj and Cebeci, Tuncer},
  year={1967},
  publisher={Douglas Aircraft Company, Douglas Aircraft Division}
}

@inproceedings{baldwin1978thin,
  title={Thin-layer approximation and algebraic model for separated turbulentflows},
  author={Baldwin, Barrett and Lomax, Harvard},
  booktitle={16th aerospace sciences meeting},
  pages={257},
  year={1978}
}


@article{maeder2001direct,
  title={Direct simulation of turbulent supersonic boundary layers by an extended temporal approach},
  author={Maeder, Thierry and Adams, Nikolaus A and Kleiser, Leonhard},
  journal={Journal of Fluid Mechanics},
  volume={429},
  pages={187--216},
  year={2001},
  publisher={Cambridge University Press}
}


@article{xin2006direct,
  title={Direct numerical simulation of a spatially evolving supersonic turbulent boundary layer at Ma= 6},
  author={Xin-Liang, Li and De-Xun, Fu and Yan-Wen, Ma},
  journal={Chinese Physics Letters},
  volume={23},
  number={6},
  pages={1519},
  year={2006},
  publisher={IOP Publishing}
}

@article{duan2010direct,
  title={Direct numerical simulation of hypersonic turbulent boundary layers. Part 2. Effect of wall temperature},
  author={Duan, Lian and Beekman, I and Martin, MP},
  journal={Journal of Fluid Mechanics},
  volume={655},
  pages={419--445},
  year={2010},
  publisher={Cambridge University Press}
}

@article{duan2011direct,
  title={Direct numerical simulation of hypersonic turbulent boundary layers. Part 3. Effect of Mach number},
  author={Duan, Lian and Beekman, I and Martin, MP},
  journal={Journal of Fluid Mechanics},
  volume={672},
  pages={245--267},
  year={2011},
  publisher={Cambridge University Press}
}

@article{chu2013effect,
  title={Effect of wall temperature on hypersonic turbulent boundary layer},
  author={Chu, You-Biao and Zhuang, Yue-Qing and Lu, Xi-Yun},
  journal={Journal of Turbulence},
  volume={14},
  number={12},
  pages={37--57},
  year={2013},
  publisher={Taylor \& Francis}
}

@article{liang2012dns,
  title={DNS and analysis of a spatially evolving hypersonic turbulent boundary layer over a flat plate at Mach 8},
  author={Liang, Xian},
  journal={SCIENTIA SINICA Physica, Mechanica \& Astronomica},
  volume={42},
  number={3},
  pages={282},
  year={2012}
}

@article{liang2013dns,
  title={DNS of a spatially evolving hypersonic turbulent boundary layer at Mach 8},
  author={Liang, Xian and Li, XinLiang},
  journal={Science China Physics, Mechanics and Astronomy},
  volume={56},
  pages={1408--1418},
  year={2013},
  publisher={Springer}
}

@article{duan2016pressure,
  title={Pressure fluctuations induced by a hypersonic turbulent boundary layer},
  author={Duan, Lian and Choudhari, Meelan M and Zhang, Chao},
  journal={Journal of Fluid Mechanics},
  volume={804},
  pages={578--607},
  year={2016},
  publisher={Cambridge University Press}
}

@article{zhang2017effect,
  title={Effect of wall cooling on boundary-layer-induced pressure fluctuations at Mach 6},
  author={Zhang, Chao and Duan, Lian and Choudhari, Meelan M},
  journal={Journal of Fluid Mechanics},
  volume={822},
  pages={5--30},
  year={2017},
  publisher={Cambridge University Press}
}

@article{zhang2018direct,
  title={Direct numerical simulation database for supersonic and hypersonic turbulent boundary layers},
  author={Zhang, Chao and Duan, Lian and Choudhari, Meelan M},
  journal={AIAA journal},
  volume={56},
  number={11},
  pages={4297--4311},
  year={2018},
  publisher={American Institute of Aeronautics and Astronautics}
}


@article{duan2012study,
  title={Study of turbulence-radiation interaction in hypersonic turbulent boundary layers},
  author={Duan, Lian and Martin, MP and Feldick, AM and Modest, MF and Levin, DA},
  journal={AIAA journal},
  volume={50},
  number={2},
  pages={447--453},
  year={2012}
}

@article{trettel2016mean,
  title={Mean velocity scaling for compressible wall turbulence with heat transfer},
  author={Trettel, Andrew and Larsson, Johan},
  journal={Physics of Fluids},
  volume={28},
  number={2},
  year={2016},
  publisher={AIP Publishing}
}

@article{griffin2021velocity,
  title={Velocity transformation for compressible wall-bounded turbulent flows with and without heat transfer},
  author={Griffin, Kevin Patrick and Fu, Lin and Moin, Parviz},
  journal={Proceedings of the National Academy of Sciences},
  volume={118},
  number={34},
  pages={e2111144118},
  year={2021},
  publisher={National Acad Sciences}
}

@article{zhang2014generalized,
  title={A generalized Reynolds analogy for compressible wall-bounded turbulent flows},
  author={Zhang, You-Sheng and Bi, Wei-Tao and Hussain, Fazle and She, Zhen-Su},
  journal={Journal of Fluid Mechanics},
  volume={739},
  pages={392--420},
  year={2014},
  publisher={Cambridge University Press}
}

@book{walz1969,
  title={Boundary layers of flow and temperature},
  author={Walz, Alfred},
  year={1969},
  publisher={Cambridge, MA: MIT Press}
}


@inproceedings{mcdonald1968extended,
  title={An extended mixing length approach for computing the turbulent boundary layer development},
  author={McDonald, Henry and Camarata, FJ},
  booktitle={Proceedings, Stanford Conference on Computation of Turbulent Boundary Layers},
  volume={1},
  pages={83--98},
  year={1968}
}


@article{menter1997eddy,
  title={Eddy Viscosity Transport Equations and Their Relation to the k-$\varepsilon$ Model},
  author={Menter, FR},
  journal={Journal of Fluids Engineering},
  volume={119},
  number={4},
  pages={876--884},
  year={1997},
  publisher={ASME International}
}

@inproceedings{bosco2011investigation,
  title={Investigation of a compression corner at hypersonic conditions using a reynolds stress model},
  author={Bosco, Arianna and Reinartz, Birgit and Brown, Laurie and Boyce, Russell},
  booktitle={17th AIAA International Space Planes and Hypersonic Systems and Technologies Conference},
  pages={2217},
  year={2011}
}

@article{frauholz2014investigation,
  title={Investigation of hypersonic intakes using Reynolds stress modeling and wavelet-based adaptation},
  author={Frauholz, Sarah and Bosco, Arianna and Reinartz, Birgit U and M{\"u}ller, Siegfried and Behr, Marek},
  journal={AIAA journal},
  volume={52},
  number={12},
  pages={2765--2781},
  year={2014},
  publisher={American Institute of Aeronautics and Astronautics}
}


@inproceedings{eisfeld2005advanced,
  title={Advanced turbulence modelling and stress analysis for the DLR-F6 configuration},
  author={Eisfeld, Bernhard and Brodersen, Olaf},
  booktitle={23rd AIAA Applied Aerodynamics Conference},
  pages={4727},
  year={2005}
}

@article{gerolymos2012term,
  title={Term-by-term analysis of near-wall second-moment closures},
  author={Gerolymos, GA and Lo, C and Vallet, I and Younis, BA},
  journal={AIAA journal},
  volume={50},
  number={12},
  pages={2848--2864},
  year={2012}
}

@article{gerolymos2002wall,
  title={Wall-normal-free near-wall Reynolds-stress model for 3-D turbomachinery flows},
  author={Gerolymos, GA and Vallet, I},
  journal={AIAA Journal},
  volume={40},
  number={2},
  pages={199208},
  year={2002}
}


@article{gerolymos2004contribution,
  title={Contribution to single-point closure Reynolds-stress modelling of inhomogeneous flow},
  author={Gerolymos, Georges A and Sauret, Emilie and Vallet, I},
  journal={Theoretical and Computational Fluid Dynamics},
  volume={17},
  pages={407--431},
  year={2004},
  publisher={Springer}
}

@techreport{speziale1989preliminary,
  title={A preliminary compressible second-order closure model for high speed flows},
  author={Speziale, Charles G and Sarkar, Sutanu},
  year={1989}
}

@article{grasso1993high,
  title={High-speed turbulence modeling of shock-wave/boundary-layer interaction},
  author={Grasso, F and Falconi, D},
  journal={AIAA journal},
  volume={31},
  number={7},
  pages={1199--1206},
  year={1993}
}

@article{van1956problem,
  title={The Problem of Aerodynamic Heating},
  author={VAN DRIEST, ER},
  journal={Aeronaut. Eng. Rev.},
  volume={15},
  number={10},
  pages={26--41},
  year={1956}
}

@inproceedings{neeb2015experimental,
  title={Experimental flow characterization and heat flux augmentation analysis of a hypersonic turbulent boundary layer along a rough surface},
  author={Neeb, Dominik and Saile, Dominik and G{\"u}lhan, Ali},
  booktitle={Proceedings of the 8th European Symposium on Aerothermodynamics for Space Vehicles},
  number={89873},
  pages={1--15},
  year={2015}
}

@article{helm2022large,
  title={Large eddy simulation of two separated hypersonic shock/turbulent boundary layer interactions},
  author={Helm, Clara M and Mart{\'\i}n, MP},
  journal={Physical Review Fluids},
  volume={7},
  number={7},
  pages={074601},
  year={2022},
  publisher={APS}
}

@article{spalding1964drag,
  title={The drag of a compressible turbulent boundary layer on a smooth flat plate with and without heat transfer},
  author={Spalding, DB and Chi, SW},
  journal={Journal of Fluid Mechanics},
  volume={18},
  number={1},
  pages={117--143},
  year={1964},
  publisher={Cambridge University Press}
}


@article{white1972simple,
  title={A simple theory for the two-dimensional compressible turbulent boundary layer},
  author={White, FM and Christoph, GH},
  journal={Journal of Fluids Engineering, Transactions of the ASME},
  volume={94},
  number={3},
  pages={636},
  year={1972}
}

@article{hopkins1971evaluation,
  title={An evaluation of theories for predicting turbulent skin friction andheat transfer on flat plates at supersonic and hypersonic Mach numbers},
  author={Hopkins, Edward J and Inouye, Mamoru},
  journal={AIAA Journal},
  volume={9},
  number={6},
  pages={993--1003},
  year={1971}
}


@inproceedings{holden1972shock,
  title={Shock wave-turbulent boundary layer interaction in hypersonic flow},
  author={HOLDEN, MS},
  booktitle={10th Aerospace Sciences Meeting},
  year={1972},
  organization={American Institute of Aeronautics and Astronautics}
}

@inproceedings{watson1973measurements,
  title={Measurements in a transitional/turbulent Mach 10 boundary layer at high-Reynolds numbers},
  author={Watson, R and Harris, J and ANDERS, JR, J},
  booktitle={11th Aerospace Sciences Meeting},
  pages={165},
  year={1973}
}

@book{winkler1959investigation,
  title={Investigation of flat plate hypersonic turbulent boundary layers with heat transfer at a Mach number of 5.2},
  author={Winkler, Ava M and Cha, Moon H},
  year={1959},
  publisher={NAVORD}
}

@article{winkler1961investigation,
  title={Investigation of Flat-Plate Hypersonic, Turbulent Boundary Layers With Heat Transfer},
  author={Winkler, Eva M},
  journal={Journal of Applied Mechanics},
  volume={28},
  number={3},
  pages={323},
  year={1961}
}

@techreport{young1965experimental,
  title={Experimental investigation of the effects of surface roughness on compressible turbulent boundary layer skin friction and heat transfer},
  author={Young, Frank Levi},
  year={1965},
  institution={Technical Report DLR-532, CR-
21 Defense Research Laboratory, University of Texas, Austin}
}

@article{heronimus1966hypersonic,
  title={Hypersonic shock tunnel experiments on the W7 flat plate model-expansion side, turbulent flow and leading edge transpiration data},
  author={Heronimus, GA},
  journal={CAL Report No. AA-1952-Y-2 (Contract No. AF 33 (615)-1847), Cornell Aeronautical Lab},
  year={1966}
}

@book{cary1970summary,
  title={Summary of available information on Reynolds analogy for zero-pressure-gradient, compressible, turbulent-boundary-layer flow},
  author={Cary, Aubrey M},
  year={1970},
  publisher={NASA TN D-5560}
}


@article{suraweera2006reynolds,
  title={Reynolds analogy in high-enthalpy and high-Mach-number turbulent flows},
  author={Suraweera, MV and Mee, DJ and Stalker, RJ},
  journal={AIAA journal},
  volume={44},
  number={4},
  pages={917--919},
  year={2006}
}

@techreport{neal1966study,
  title={A study of the pressure, heat transfer, and skin friction on sharp and blunt flat plates at Mach 6.8},
  author={Neal Jr, Luther},
  year={1966},
  publisher={Technical Note D-3312 (Washington, DC: National Aeronautics and Space Administration)}
}

@article{danberg1964characteristics,
  title={Characteristics of the turbulent boundary layer with heat and mass transfer at M= 6.7},
  author={Danberg, James Edward},
  year={1964},
  publisher={Technical Report NOLTR 64-99 (White Oak, Silver Spring, MD: United States Naval Ordnance Laboratory)}
}

@article{danberg1967characteristics,
  title={Characteristics of the turbulent boundary layer with heat and mass transfer: data tabulation},
  author={Danberg, James E},
  journal={NOLTR 675-6},
  year={1967}
}


@article{wallace1967hypersonic,
  title={Hypersonic Turbulent Boundary Layer Studies at Cold Wall Temperatures},
  author={Wallace, J},
  journal={Proceedings of the 1967 Heat Transfer and Fluid Mechanics Institute held at the University of California, San Diego, La Jolla, California},
  year={1967}
}

@article{keener1972measurements,
  title={Measurements of Reynolds analogy for a hypersonic turbulent boundary layer on a nonadiabatic flat plate},
  author={Keener, Earl R and Polek, Thomas E},
  journal={AIAA Journal},
  volume={10},
  number={6},
  pages={845--846},
  year={1972}
}

@techreport{voisinet1972measurements,
  title={Measurements of a Mach 4.9 zero-pressure-gradient turbulent boundary layer with heat transfer. Part 1: Data compilation},
  author={Voisinet, RLP and Lee, Roland E},
  year={1972},
  institution={Technical Report NOLTR 72-232 (White Oak, Silver Spring, MD: United States Naval Ordnance Laboratory)}
}

@article{hill1956boundary,
  title={Boundary-layer measurements in hypersonic flow},
  author={Hill, FK},
  journal={Journal of the Aeronautical Sciences},
  volume={23},
  number={1},
  pages={35--42},
  year={1956}
}

@book{lee1969velocity,
  title={Velocity Profile, Skin-friction Balance and Heat-transfer Measurements of the Turbulent Boundary Layers at Mach 5 and Zero-pressure Gradient},
  author={Lee, Roland E and Yanta, William Joseph and Leonas, Annette C},
  volume={69},
  year={1969},
  publisher={United States Naval Ordnance Laboratory}
}

@book{matting1961turbulent,
  title={Turbulent skin friction at high Mach numbers and Reynolds numbers in air and helium},
  author={Matting, Fred W},
  volume={82},
  year={1961},
  publisher={National Aeronautics and Space Administration}
}

@article{laderman1974mean,
  title={Mean and fluctuating flow measurements in the hypersonic boundary layer over a cooled wall},
  author={Laderman, AJ and Demetriades, A},
  journal={Journal of Fluid Mechanics},
  volume={63},
  number={1},
  pages={121--144},
  year={1974},
  publisher={Cambridge University Press}
}

@inproceedings{backx1973measurements,
  title={Measurements in the Mach 15 turbulent boundary layer on the wall of the longshot conical nozzle},
  booktitle={EUROMECH, Colloquium on Heat Transfer in Turbulent Boundary Layers with Variable Fluid Properties, Goettingen, West Germany},
  author={Backx, Edgard},
  year={1973}
}

@article{backx1974experimental,
  title={Experimental study of the turbulent boundary layer at Mach 15 and 19. 8 in a conical nozzle},
  author={Backx, Edgard},
  year={1974},
  publisher={Technical Note 102 von Kármán Institute for Fluid Dynamics}
}

@article{backx1976high,
  title={A high Mach Number turbulent boundary-layer study},
  author={Backx, E and Richards, BE},
  journal={AIAA Journal},
  volume={14},
  number={9},
  pages={1159--1160},
  year={1976}
}

@article{horstman1972turbulent,
  title={Turbulent properties of a compressible boundary layer.},
  author={Horstman, CC and Owen, FK},
  journal={AIAA Journal},
  volume={10},
  number={11},
  pages={1418--1424},
  year={1972}
}

@article{owen1972structure,
  title={On the structure of hypersonic turbulent boundary layers},
  author={Owen, FK and Horstman, CC},
  journal={Journal of Fluid Mechanics},
  volume={53},
  number={4},
  pages={611--636},
  year={1972},
  publisher={Cambridge University Press}
}


@article{murray2013experimental,
  title={Experimental investigation of axisymmetric hypersonic shock-wave/turbulent-boundary-layer interactions},
  author={Murray, N and Hillier, R and Williams, S},
  journal={Journal of Fluid Mechanics},
  volume={714},
  pages={152--189},
  year={2013},
  publisher={Cambridge University Press}
}


@book{samuels1967experimental,
  title={Experimental investigation of the turbulent boundary layer at a Mach number of 6 with heat transfer at high Reynolds numbers},
  author={Samuels, Richard D and Peterson, John B and Adcock, Jerry B},
  volume={3858},
  year={1967},
  publisher={National Aeronautics and Space Administration}
}

@article{sciacovelli2020numerical,
  title={Numerical investigation of high-speed turbulent boundary layers of dense gases},
  author={Sciacovelli, Luca and Gloerfelt, Xavier and Passiatore, Donatella and Cinnella, Paola and Grasso, Francesco},
  journal={Flow, Turbulence and Combustion},
  volume={105},
  pages={555--579},
  year={2020},
  publisher={Springer}
}


@techreport{kussoy1975experimental,
  title={An experimental documentation of a hypersonic shock-wave turbulent boundary layer interaction flow: With and without separation},
  author={Kussoy, MI and Horstmann, CC},
  year={1975}
}

@article{appels1973turbulent,
  title={Turbulent boundary layer separation at Mach 12},
  author={Appels, C},
  journal={VKI TN-90},
  year={1973}
}

@article{coet1993experiments,
  title={Experiments on shock wave/boundary layer interaction in hypersonic flow},
  author={COET, MARIE-},
  journal={La Recherche Aerospatiale(English Edition)},
  number={1},
  pages={61--74},
  year={1993}
}


@article{kussoy1993hypersonic,
  title={Hypersonic crossing shock-wave/turbulent-boundary-layer interactions},
  author={Kussoy, MI and Horstoman, KC and Horstman, C},
  journal={AIAA journal},
  volume={31},
  number={12},
  pages={2197--2203},
  year={1993}
}

@article{coleman1973study,
  title={A study of hypersonic boundary layers over a family of axisymmetric bodies at zero incidence: preliminary report and data tabulation},
  author={Coleman, GT},
  journal={Imperial College Aero Report 73-06 Imperial College of Science and Technology, London, UK},
  year={1973}
}

@phdthesis{coleman1973hypersonic,
  title={Hypersonic turbulent boundary layer studies},
  author={Coleman, Graham Trevor},
  year={1973},
  school={Imperial College London}
}

@article{coleman1974incipient,
  title={Incipient separation of axially symmetric hypersonic turbulent boundary layers},
  author={Coleman, GT and Stollery, JL},
  journal={AIAA Journal},
  volume={12},
  number={1},
  pages={119--120},
  year={1974}
}


@article{holden2014measurements,
  title={Measurements in Regions of Shock Wave/Turbulent Boundary Layer Interaction on Double cone and Hollow Cylinder/Flare Configurations for Open and},
  author={Holden, M and Wadhams, T and MacLean, M},
  journal={Blind” Code Evaluation/Validation,” Tech. rep., American Institute of Aeronautics and Astronautics},
  year={2014}
}


@inproceedings{holden2018measurements,
  title={Measurements in regions of shock wave/turbulent boundary layer interaction from Mach 4 to 7 at flight duplicated velocities to evaluate and improve the models of turbulence in CFD codes},
  author={Holden, Michael},
  booktitle={2018 Fluid Dynamics Conference},
  pages={3706},
  year={2018}
}

@article{running2019hypersonic,
  title={Hypersonic shock-wave/boundary-layer interactions on a cone/flare},
  author={Running, Carson L and Juliano, Thomas J and Jewell, Joseph S and Borg, Matthew P and Kimmel, Roger L},
  journal={Experimental Thermal and Fluid Science},
  volume={109},
  pages={109911},
  year={2019},
  publisher={Elsevier}
}


@article{borovoy2009laminar,
  title={Laminar-turbulent flow over wedges mounted on sharp and blunt plates},
  author={Borovoy, V Ya and Mosharov, VN and Noev, A Yu and Radchenko, VN},
  journal={Fluid Dynamics},
  volume={44},
  number={3},
  pages={382--396},
  year={2009},
  publisher={Springer}
}

@article{borovoy20123d,
  title={3D shock/turbulent boundary layer interaction on the plate near a wedge in presence of an entropy layer},
  author={Borovoy, Volf Ya and Egorov, Ivan Vladimirovich and Noev, Anton Yurievich and Radchenko, Vladimir Nikolaevich and Skuratov, Arkadii Sergeyevich and Struminskaya, Irina Vladimirovna},
  journal={TsAGI Science Journal},
  volume={43},
  number={6},
  year={2012},
  publisher={Begel House Inc.}
}

@article{borovoy2016entropy,
  title={Entropy-layer influence on single-fin and double-fin/boundary-layer interactions},
  author={Borovoy, Volf and Egorov, Ivan and Mosharov, Vladimir and Radchenko, Vladimir and Skuratov, Arkady and Struminskaya, Irina},
  journal={AIAA Journal},
  volume={54},
  number={2},
  pages={443--457},
  year={2016},
  publisher={American Institute of Aeronautics and Astronautics}
}

@book{law1975three,
  title={Three-dimensional shock wave-turbulent boundary layer interactions at Mach 6},
  author={Law, C Herbert},
  volume={75},
  number={191},
  year={1975},
  publisher={Aerospace Research Laboratories, Air Force Systems Command, United States~…}
}


@inproceedings{rodi1992experimental,
  title={An experimental/computational study of sharp fin induced shock wave/turbulent boundary layer interactions at Mach 5-Experimental results},
  author={RODI, PATRICK and DOLLING, DAVID},
  booktitle={30th Aerospace Sciences Meeting and Exhibit},
  pages={749},
  year={1992}
}


@article{rodi1995behavior,
  title={Behavior of pressure and heat transfer in sharp fin-induced turbulent interactions},
  author={Rodi, PE and Dolling, DS},
  journal={AIAA journal},
  volume={33},
  number={11},
  pages={2013--2019},
  year={1995}
}

@inproceedings{rodi1991experimental,
  title={An experimental/computational study of heat transfer in sharp fin induced turbulent interactions at Mach 5},
  author={Rodi, P and Dolling, D and KNIGHT, DOYLED},
  booktitle={22nd Fluid Dynamics, Plasma Dynamics and Lasers Conference},
  pages={1764},
  year={1991}
}


@inproceedings{holden1984experimental,
  title={Experimental studies of quasi-two-dimensional and three-dimensional viscous interaction regions induced by skewed-shock and swept-shock boundary layer interaction},
  author={Holden, M},
  booktitle={17th Fluid Dynamics, Plasma Dynamics, and Lasers Conference},
  pages={1677},
  year={1984}
}


@book{hopkins1969summary,
  title={Summary and correlation of skin-friction and heat-transfer data for a hypersonic turbulent boundary layer on simple shapes},
  author={Hopkins, Edward J},
  volume={5089},
  year={1969},
  publisher={National Aeronautics and Space Administration}
}


@book{hopkins1970direct,
  title={Direct Measurements of Turbulent Skin Friction on a Nonadiabatic Flat Plate at Mach Number 6.5 and Comparisons With Eight Theories},
  author={Hopkins, Edward J},
  year={1970},
  publisher={National Aeronautics and Space Administration}
}


@article{hopkins1972hypersonic,
  title={Hypersonic turbulent skin-friction and boundary-layer profiles on nonadiabatic flat plates},
  author={Hopkins, Edward J and Keener, Earl R and Polek, Thomas E and Dwyer, Harry A},
  journal={AIAA Journal},
  volume={10},
  number={1},
  pages={40--48},
  year={1972}
}

@article{hill1959turbulent,
  title={Turbulent boundary layer measurements at Mach numbers from 8 to 10},
  author={Hill, FK},
  journal={The Physics of Fluids},
  volume={2},
  number={6},
  pages={668--680},
  year={1959},
  publisher={American Institute of Physics}
}


@article{roy2018variable,
  title={Variable turbulent Prandtl number model for shock/boundary-layer interaction},
  author={Roy, Subhajit and Pathak, Utkarsh and Sinha, Krishnendu},
  journal={AIAA Journal},
  volume={56},
  number={1},
  pages={342--355},
  year={2018},
  publisher={American Institute of Aeronautics and Astronautics}
}


@article{guo2023amplification,
  title={Amplification of turbulent kinetic energy and temperature fluctuation in a hypersonic turbulent boundary layer over a compression ramp},
  author={Guo, Tongbiao and Zhang, Ji and Tong, Fulin and Li, Xinliang},
  journal={Physics of Fluids},
  volume={35},
  number={4},
  year={2023},
  publisher={AIP Publishing}
}


@article{collen2021development,
  title={Development and commissioning of the T6 Stalker Tunnel},
  author={Collen, Peter and Doherty, Luke J and Subiah, Suria D and Sopek, Tamara and Jahn, Ingo and Gildfind, David and Penty Geraets, Rowland and Gollan, Rowan and Hambidge, Christopher and Morgan, Richard and others},
  journal={Experiments in Fluids},
  volume={62},
  pages={1--24},
  year={2021},
  publisher={Springer}
}

@article{kimmel1997effect,
  title={The effect of pressure gradients on transition zone length in hypersonic boundary layers},
  author={KIMMEL, RL},
  journal={Journal of fluids engineering},
  volume={119},
  number={1},
  pages={36--41},
  year={1997}
}

@article{kimmel1993experimental,
  title={Experimental transition zone lengths in pressure gradient in hypersonic flow},
  author={Kimmel, RL},
  journal={ASME-PUBLICATIONS-FED},
  volume={151},
  pages={117--117},
  year={1993},
  publisher={ASME}
}


@article{babinsky1997large,
  title={Large-scale roughness influence on turbulent hypersonic boundary layers approaching compression corners},
  author={Babinsky, H and Edwards, JA},
  journal={Journal of spacecraft and rockets},
  volume={34},
  number={1},
  pages={70--75},
  year={1997}
}









%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%JPH%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


@article{Chen_Donzis_2019, title={Shock–turbulence interactions at high turbulence intensities}, volume={870}, rights={https://www.cambridge.org/core/terms}, ISSN={0022-1120, 1469-7645}, DOI={10.1017/jfm.2019.248}, abstractNote={Shock–turbulence interactions are investigated using well-resolved direct numerical simulations (DNS) and analysis at a range of Reynolds, mean and turbulent Mach numbers (Rλ, M and Mt, respectively). The simulations are shock and turbulence resolving with Rλ up to 65, Mt up to 0.54 and M up to 1.4. The focus is on the effect of strong turbulence on the jumps of mean thermodynamic variables across the shock, the shock structure and the ampliﬁcation of turbulence as it moves through the shock. Theoretical results under the so-called quasi-equilibrium (QE) assumption provide explicit laws for a number of statistics of interests which are in agreement with the new DNS data presented here as well as all the data available in the literature. While in previous studies turbulence was found to weaken jumps, it is shown here that stronger jumps are also observed depending on the regime of the interaction. Statistics of the dilatation at the shock are also investigated and found to be well represented by QE for weak turbulence but saturate at high turbulence intensities with a Reynolds number dependence also captured by the analysis. Finally, ampliﬁcation factors are found to present a universal behaviour with two limiting asymptotic regimes governed by (M − 1) and K = Mt/R1λ/2(M − 1), for weak and strong turbulence, respectively. Effect of anisotropy in the incoming ﬂow is also assessed by utilizing two different forcing mechanisms to generate turbulence.}, journal={Journal of Fluid Mechanics}, author={Chen, Chang Hsin and Donzis, Diego A.}, year={2019}, month=jul, pages={813–847}, language={en} }

 @article{Larsson_Bermejo-Moreno_Lele, title={Reynolds- and Mach-number eﬀects in canonical shock–turbulence interaction}, volume={717}, DOI={10.1017/jfm.2012.573}, journal={Journal of Fluid Mechanics}, author={Larsson, Johan and Bermejo-Moreno, Ivan and Lele, Sanjiva K.}, year={2013}, pages={293–321}}


 @book{Ribner_1954, title={Convection of a pattern of vorticity through a shock wave}, abstractNote={An arbitrary weak spatial distribution of vorticity can be represented in terms of plane sinusoidal shear waves of all orientations and wave lengths. (Fourier integral). The analysis treats the passage of a single representative weak shear wave through a plane shock and shows refraction and modijication of the shear wave with simultaneous generation of an acoustically.}, number={1164}, institution={NACA}, author={Ribner, H S}, year={1954}, language={en} }


 @article{Lele_1992, title={Shock-jump relations in a turbulent flow}, volume={4}, ISSN={0899-8213}, DOI={10.1063/1.858343}, abstractNote={The exact jump relations applying across a shock in turbulent mean flow are formulated. These are analyzed to obtain answers to the following basic questions: Is the propagation speed of a shock wave which brings about a specified compression faster or slower than its classical value when moving through a turbulent medium? What is the magnitude of the turbulence associated correction? What is the magnitude of the correction to the pressure jump? Answers to these questions are developed by combining gas-dynamic analysis with homogeneous rapid distortion approximation.}, number={12}, journal={Physics of Fluids A: Fluid Dynamics}, author={Lele, Sanjiva K.}, year={1992}, month=dec, pages={2900–2905}, language={en} }

 @article{Yang_Wang_Gao_2022, title={Studies on effects of wall temperature variation on heat transfer in hypersonic laminar boundary layer}, volume={190}, ISSN={00179310}, DOI={10.1016/j.ijheatmasstransfer.2022.122790}, journal={International Journal of Heat and Mass Transfer}, author={Yang, Zepeng and Wang, Suozhu and Gao, Zhenxun}, year={2022}, month=jul, pages={122790}, language={en} }


 @article{prasad2023turbulence,
  title={Turbulence modeling of 3D high-speed flows with upstream-informed corrections},
  author={Prasad, Chitrarth and Gaitonde, Datta V},
  journal={Shock Waves},
  volume={33},
  number={2},
  pages={99--115},
  year={2023},
  publisher={Springer}
}

 @article{Karl_Bykerk_2024, title={Sustainable space technologies—Strategies toward a predictive aerothermal design of re-useable space transportation systems}, volume={95}, ISSN={0034-6748, 1089-7623}, DOI={10.1063/5.0177075}, abstractNote={This paper presents a review of current aerothermal design and analysis methodologies for spacecraft. It briefly introduces the most important system architectures, including rockets, gliders, and capsule-based configurations, and gives an overview of the specific aerothermal and thermo-chemical effects that are encountered during their different flight phases and trajectories. Numerical and experimental design tools of different fidelity levels are reviewed and discussed, with a specific focus placed on the present limitations and uncertainty sources of models for the wide range of physical phenomena that are encountered in the analyses. This includes high temperature thermodynamics, chemical effects, turbulence, radiation, and gasdynamic effects. This is followed by a summary of current predictive capabilities and research foci, with missing capabilities identified. Finally, a future strategy toward an efficient and predictive aerothermal design of re-useable space transportation systems is proposed.}, number={2}, journal={Review of Scientific Instruments}, author={Karl, Sebastian and Bykerk, Tamas}, year={2024}, month=feb, pages={021101}, language={en} }


 @article{Griffond_Soulard_2012, title={Evolution of axisymmetric weakly turbulent mixtures interacting with shock or rarefaction waves}, volume={24}, ISSN={1070-6631, 1089-7666}, DOI={10.1063/1.4767729}, abstractNote={This paper deals with the interaction of a shock or a rarefaction wave with a weakly turbulent mixture of perfect gases. Assuming weak density-velocity fluctuations, Kovasznay decomposition applies and linear theories can be used to predict the evolution of the joint spectrum of density and velocity during the interaction. In this work, the upstream spectrum is restricted to axisymmetric fields free of acoustic perturbations, in order to comply with shock tube experimental conditions. Besides, spectral anisotropy is limited to a first order spherical harmonic decomposition. With these assumptions, transfer matrices can be obtained which relate the Reynolds stresses, turbulent mass flux and density variance after interaction to their counterparts before interaction. Results are given for both shock waves and rarefaction or compression waves; they are intended to help improve one-point statistical turbulence models applied to shock tube experiments.}, number={11}, journal={Physics of Fluids}, author={Griffond, Jérôme and Soulard, Olivier}, year={2012}, month=nov, pages={115108}, language={en} }


 @article{Tian_Gao_Jiang_Lee_2023, title={A correction for Reynolds‐averaged‐Navier–Stokes turbulence model under the effect of shock waves in hypersonic flows}, volume={95}, ISSN={0271-2091, 1097-0363}, DOI={10.1002/fld.5150}, abstractNote={Studies on the unphysical increase of turbulent quantities for RANS simulation induced by shock waves in hypersonic flows are carried out. Numerical experiments on the hypersonic flow over a blunt body reveal that the phenomenon of unphysical increase of turbulent quantities across the detached shock wave is induced by the strain-rate-based production terms of the k-�� and k-�� SST turbulence models, which leads to the over-prediction of aerothermal prediction. While this phenomenon does not occur for Spalart–Allmaras (S–A) turbulence model because of its vorticity-based production term. In order to eliminate this unphysical phenomenon, and to maintain the accuracy of the original models for boundary layer and separation flows, a new correction method for the k-�� and k-�� SST models is proposed: by comparing the orders of magnitude between the strain-rate-based and vorticity-based production terms, the vorticity-based production term is used near the shock waves, while the original strain-rate-based production term is still used in other regions. Finally, the correction method is applied to turbulence and transition flows over blunt bodies, and the numerical results show that the correction method effectively eliminates the unphysical increase of turbulent quantities across shock waves and improves the accuracy of aerothermal and transition onset location prediction.}, number={2}, journal={International Journal for Numerical Methods in Fluids}, author={Tian, Yuyan and Gao, Zhenxun and Jiang, Chongwen and Lee, Chun‐Hian}, year={2023}, month=feb, pages={313–333}, language={en} }


 @article{Zhang_Gao_Jiang_Lee_2017, title={A RANS model correction on unphysical over-prediction of turbulent quantities across shock wave}, volume={106}, ISSN={00179310}, DOI={10.1016/j.ijheatmasstransfer.2016.10.087}, abstractNote={The unphysical increase of turbulent quantities in turbulence model induced by shock wave in simulations of hypersonic ﬂows and its inﬂuence on the aerothermal prediction are studied. Using k-x SST model, numerical experiments on the hypersonic ﬂow over a blunt body indicate that the strong detached shock wave will result in serious unphysical increase of turbulent quantities and the increase magnitudes are closely related to the mesh scales near the shock wave. This phenomenon could generally cause an over-prediction of the aerothermal prediction. To eliminate this unphysical phenomenon and enhance the accuracy of aerothermal prediction, a new correction model for current k-x SST model is established, which includes two parts: a shock wave detector to identify the location of shock wave and a damping function for the production terms in turbulent transport equations. Finally, the modiﬁed k-x SST model using the correction model is applied to two types of hypersonic ﬂows. Numerical results prove that the correction model can effectively eliminate the unphysical increase of turbulent quantities around the shock wave and meanwhile does not affect the normal development of turbulent quantities inside boundary layer. Through the correction model, the accuracy of aerothermal prediction is remarkably improved.}, journal={International Journal of Heat and Mass Transfer}, author={Zhang, Zhichao and Gao, Zhenxun and Jiang, Chongwen and Lee, Chun-Hian}, year={2017}, month=mar, pages={1107–1119}, language={en} }


@article{Zank_Zhou_Matthaeus_Rice_2002, title={The interaction of turbulence with shock waves: A basic model}, volume={14}, ISSN={1070-6631, 1089-7666}, DOI={10.1063/1.1507772}, abstractNote={The interaction of turbulence and shock waves is considered self-consistently so that the back-reaction of the turbulence and its associated reaction on the turbulence is addressed. This approach differs from previous studies which considered the interaction of linear modes with a shock. The most basic model of hypersonic flow, described by the inviscid form of Burgers’ equation, is used. An energy-containing model which couples the turbulent energy density and correlation length of the flow with the mean flow is developed. Upstream turbulence interacting with a shock wave is found to mediate the shock by (1) increasing the mean shock speed, and (2) decreasing the efficiency of turbulence amplification at the shock as the upstream turbulence energy density is increased. The implication of these results is that the energy in upstream turbulent fluctuations, while being amplified at the shock, is also being converted into mean flow energy downstream. The variance in both the shock speed and position is computed, leading to the suggestion that, in an ensemble-averaged sense, the turbulence mediated shock will acquire a characteristic thickness given by the standard deviation of the shock position. Lax’s geometric entropy condition is used to show that as the upstream turbulent energy density increases, the shock is eventually destabilized, and may emit one or more shocks to produce a system of multiple shock waves. Finally, turbulence downstream of the shock is shown to decay in time t according to t−2/3.}, number={11}, journal={Physics of Fluids}, author={Zank, G. P. and Zhou, Ye and Matthaeus, W. H. and Rice, W. K. M.}, year={2002}, month=nov, pages={3766–3774}, language={en} }

 @article{Chen_Donzis_2019, title={Shock–turbulence interactions at high turbulence intensities}, volume={870}, rights={https://www.cambridge.org/core/terms}, ISSN={0022-1120, 1469-7645}, DOI={10.1017/jfm.2019.248}, abstractNote={Shock–turbulence interactions are investigated using well-resolved direct numerical simulations (DNS) and analysis at a range of Reynolds, mean and turbulent Mach numbers (Rλ, M and Mt, respectively). The simulations are shock and turbulence resolving with Rλ up to 65, Mt up to 0.54 and M up to 1.4. The focus is on the effect of strong turbulence on the jumps of mean thermodynamic variables across the shock, the shock structure and the ampliﬁcation of turbulence as it moves through the shock. Theoretical results under the so-called quasi-equilibrium (QE) assumption provide explicit laws for a number of statistics of interests which are in agreement with the new DNS data presented here as well as all the data available in the literature. While in previous studies turbulence was found to weaken jumps, it is shown here that stronger jumps are also observed depending on the regime of the interaction. Statistics of the dilatation at the shock are also investigated and found to be well represented by QE for weak turbulence but saturate at high turbulence intensities with a Reynolds number dependence also captured by the analysis. Finally, ampliﬁcation factors are found to present a universal behaviour with two limiting asymptotic regimes governed by (M − 1) and K = Mt/R1λ/2(M − 1), for weak and strong turbulence, respectively. Effect of anisotropy in the incoming ﬂow is also assessed by utilizing two different forcing mechanisms to generate turbulence.}, journal={Journal of Fluid Mechanics}, author={Chen, Chang Hsin and Donzis, Diego A.}, year={2019}, month=jul, pages={813–847}, language={en} }


 @article{Jacquin_Cambon_Blin_1993, title={Turbulence amplification by a shock wave and rapid distortion theory}, volume={5}, number={10}, journal={Phys. Fluids A}, author={Jacquin, L and Cambon, C and Blin, E}, year={1993}, language={en} }

 @article{Lacombe_Roy_Sinha_Karl_Hickey_2021, title={Characteristic Scales in Shock–Turbulence Interaction}, volume={59}, ISSN={0001-1452, 1533-385X}, DOI={10.2514/1.J059499}, number={2}, journal={AIAA Journal}, author={Lacombe, Francis and Roy, Subhajit and Sinha, Krishnendu and Karl, Sebastian and Hickey, Jean-Pierre}, year={2021}, month=feb, pages={526–532}, language={en} }


@article{SuSi19,
	author = {Roy, Subhajit and Sinha, Krishnendu},
	doi = {10.2514/1.J058334},
	eprint = {https://doi.org/10.2514/1.J058334},
	journal = {AIAA Journal},
	number = {8},
	pages = {3624-3629},
	title = {Turbulent Heat Flux Model for Hypersonic Shock--Boundary Layer Interaction},
	url = {https://doi.org/10.2514/1.J058334},
	volume = {57},
	year = {2019},
	bdsk-url-1 = {https://doi.org/10.2514/1.J058334}}



 @article{Sinha_Mahesh_Candler_2003, title={Modeling shock unsteadiness in shock/turbulence interaction}, volume={15}, ISSN={1070-6631, 1089-7666}, DOI={10.1063/1.1588306}, abstractNote={The RANS (Reynolds averaged Navier–Stokes) equations can yield significant error when applied to practical flows involving shock waves. We use the interaction of homogeneous isotropic turbulence with a normal shock to suggest improvements in the k–ε model applied to shock/turbulence interaction. Mahesh et al. [J. Fluid Mech. 334, 353 (1997)] and Lee et al. [J. Fluid Mech. 340, 22 (1997)] present direct numerical simulation (DNS) and linear analysis of the flow of isotropic turbulence through a normal shock, where it is found that mean compression, shock unsteadiness, pressure-velocity correlation, and up-stream entropy fluctuations play an important role in the interaction. Current RANS models based on the eddy viscosity assumption yield very high amplification of the turbulent kinetic energy, k, across the shock. Suppressing the eddy viscosity in a shock improves the model predictions, but is inadequate to match theoretical results at high Mach numbers. We modify the k equation to include a term due to shock unsteadiness, and model it using linear analysis. The dissipation rate equation is similarly altered based on linear analysis results. These modifications improve the model predictions considerably, and the new model is found to match the linear theory and DNS data well.}, number={8}, journal={Physics of Fluids}, author={Sinha, Krishnendu and Mahesh, Krishnan and Candler, Graham V.}, year={2003}, month=aug, pages={2290–2297}, language={en} }
 
 @article{Braun_Gore_2018, title={On primitive variable behaviour near shocks in ensemble-averaged methods}, volume={19}, abstractNote={Models for averaged shock corrugation effects and the impact of turbulent entropy or acoustic modes on the energy equation are presented, for application in Reynolds-Averaged Navier Stokes(RANS) simulations of shock-turbulence interactions. Unlike previous work that has focused the modification of turbulent statistics by the shock, the proposed models are introduced to capture the effects of the turbulence on the profiles of primitive variables - mean density, velocity, and pressure. By producing accurate profiles for the primitive variables, it is shown that the proposed models improve numerical convergence behaviour with mesh refinement about a shock, and introduce the physical effects of shock asphericity in a converging shock geometry. These effects are achieved by local closures to turbulent statistics in the averaged Navier-Stokes equations, and can be applied in conjunction with existing Reynolds stress closures that have been constructed for broader applications beyond shock-turbulence interactions.}, number={10}, journal={JOURNAL OF TURBULENCE}, author={Braun, N O and Gore, R A}, year={2018}, pages={868–888}, language={en} }




 @article{Zhang_2017, title={A RANS model correction on unphysical over-prediction of turbulent quantities across shock wave}, abstractNote={The unphysical increase of turbulent quantities in turbulence model induced by shock wave in simulations of hypersonic ﬂows and its inﬂuence on the aerothermal prediction are studied. Using k-x SST model, numerical experiments on the hypersonic ﬂow over a blunt body indicate that the strong detached shock wave will result in serious unphysical increase of turbulent quantities and the increase magnitudes are closely related to the mesh scales near the shock wave. This phenomenon could generally cause an over-prediction of the aerothermal prediction. To eliminate this unphysical phenomenon and enhance the accuracy of aerothermal prediction, a new correction model for current k-x SST model is established, which includes two parts: a shock wave detector to identify the location of shock wave and a damping function for the production terms in turbulent transport equations. Finally, the modiﬁed k-x SST model using the correction model is applied to two types of hypersonic ﬂows. Numerical results prove that the correction model can effectively eliminate the unphysical increase of turbulent quantities around the shock wave and meanwhile does not affect the normal development of turbulent quantities inside boundary layer. Through the correction model, the accuracy of aerothermal prediction is remarkably improved.}, journal={International Journal of Heat and Mass Transfer}, author={Zhang, Zhichao}, year={2017}, language={en} }


 @article{Ryu_Livescu_2014, title={Turbulence structure behind the shock in canonical shock–vortical turbulence interaction}, volume={756}, rights={https://www.cambridge.org/core/terms}, ISSN={0022-1120, 1469-7645}, DOI={10.1017/jfm.2014.477}, abstractNote={The interaction between vortical isotropic turbulence (IT) and a normal shock wave is studied using direct numerical simulation (DNS) and linear interaction analysis (LIA). In previous studies, agreement between the simulation results and the LIA predictions has been limited and, thus, the signiﬁcance of LIA has been underestimated. The results show, for the ﬁrst time, that the turbulence quantities from DNS converge to the LIA solutions as the turbulent Mach number, Mt, becomes small, even at low upstream Reynolds numbers. The classical LIA formulae are extended to compute the complete post-shock ﬂow ﬁelds using an IT database. The solutions, consistent with the DNS results, show that the shock wave signiﬁcantly changes the topology of the turbulent structures, with a symmetrization of the third invariant of the velocity gradient tensor and (Ms-mediated) of the probability density function (PDF) of the longitudinal velocity derivatives, and an Ms-dependent increase in the correlation between strain and rotation.}, journal={Journal of Fluid Mechanics}, author={Ryu, Jaiyoung and Livescu, Daniel}, year={2014}, month=oct, pages={R1}, language={en} }

@book{Howarth1953,
publisher = {Clarendon Press},
series = {The Oxford engineering science series},
title = {Modern developments in fluid dynamics : high speed flow },
booktitle = {Modern developments in fluid dynamics : high speed flow},
keywords = {Fluid dynamics},
language = {eng},
lccn = {54005834},
year = {1953},
author = {Howarth, Leslie.},
address = {Oxford},
}




 @article{Cheng_Fu_2024, title={Mean temperature scalings in compressible wall turbulence}, volume={9}, ISSN={2469-990X}, DOI={10.1103/PhysRevFluids.9.054610}, number={5}, journal={Physical Review Fluids}, author={Cheng, Cheng and Fu, Lin}, year={2024}, month=may, pages={054610}, language={en} }

 @article{Gelain2021, title={Aerothermal characterisation of a surface heat exchanger implemented in a turbofan by-pass duct}, author={Gelain, Matteo}, language={en} ,  year={2021},
  school={Universit{\'e} Paris-Saclay}}


 @inproceedings{Maheu_Moureau_Domingo_2012, title={Large-Eddy Simulations of flow and heat transfer around a low-Mach number turbine blade}, ISBN={978-1-56700-302-4}, url={http://www.dl.begellhouse.com/references/1bb331655c289a0a,7c69ce3452e09525,6e8103ad5d4ba006.html}, DOI={10.1615/ICHMT.2012.ProcSevIntSympTurbHeatTransfPal.810}, booktitle={Proceeding of THMT-12. Proceedings of the Seventh International Symposium On Turbulence, Heat and Mass Transfer Palermo, Italy, 24-27 September, 2012}, publisher={Begellhouse}, author={Maheu, Nicolas and Moureau, Vincent and Domingo, P.}, year={2012}, pages={12}, language={en} }


 @inproceedings{muller2024investigation,
  title={Investigation of Loosely-Coupled Conjugate Heat Transfer With Wall-Modeled Large Eddy Simulation in a Mach 2.5 Flow},
  author={Muller, Julia and Boisvert, Joshua and Dutta, Meghna and Oefelein, Joseph},
  booktitle={AIAA AVIATION FORUM AND ASCEND 2024},
  pages={4175},
  year={2024}
}

@inproceedings{Muller_Dutta_Boisvert_Oefelein_2024, address={London, United Kingdom}, title={Investigation of Conjugate Heat Transfer in Wall-Modeled Large Eddy Simulation of High-Speed Compressible Wall-Bounded Flows}, ISBN={978-0-7918-8809-4}, url={https://asmedigitalcollection.asme.org/GT/proceedings/GT2024/88094/V013T13A034/1204874}, DOI={10.1115/GT2024-127902}, abstractNote={A parameter study is performed in a compressible boundarylayer at supersonic conditions to investigate the accuracy of a validated loosely-coupled Conjugate Heat Transfer (CHT) model combined with an advanced wall model approach for Large Eddy Simulation (LES). Fully-coupled CHT typically introduces extreme additional cost to numerical simulations due to large timescale disparities between processes in the fluid and solid domains. Loosely-coupled CHT methods seek to mitigate this cost while simultaneously maintaining the correct boundary layer dynamics and local heat transfer processes. Likewise, wall-modeling makes LES more computationally tractable, but has not been widely used with CHT. The current investigation demonstrates the performance (accuracy and computational cost) of these approaches when implemented as a unified model. Results demonstrate that the selected wall-modeled LES, combined with a fully-integrated loosely-coupled CHT model, can reproduce the accuracy of reference DNS and wall-resolved LES data with orders of magnitude reduction in cost. Moreover, they demonstrate the implementation requirements necessary to achieve this accuracy.}, booktitle={Volume 13: Heat Transfer: General Interest / Additive Manufacturing Impacts on Heat Transfer; Wind Energy}, publisher={American Society of Mechanical Engineers}, author={Muller, Julia A. and Dutta, Meghna and Boisvert, Joshua and Oefelein, Joseph C.}, year={2024}, month=jun, pages={V013T13A034}, language={en} }

 @article{Yang_Iacovides_Craft_Apsley_2021, title={RANS Model development on temperature variance in conjugate heat transfer}, volume={22}, ISSN={1468-5248}, DOI={10.1080/14685248.2020.1860214}, abstractNote={In this study, a RANS model of turbulent conjugate heat transfer has been developed, which is applicable across a range of different combination of fluid and solid thermal properties. This is achieved by focusing on the transport equations for the temperature variance and its dissipation rate across the solid walls which bound the flow region. In this investigation we make use of a wider range of DNS data reported by other researchers, to advance our understanding of the processes involved and to revise and extend the capabilities of the model of Craft et al [12] including a more physical fluid-solid interface condition on the dissipation of thermal fluctuations and a dependence of model coefficients on Prandtl number. The resulting model is shown to successfully reproduce the penetration of thermal fluctuations into solid regions, and their subsequent decay across the solid, for a wide range of fluid to solid thermal property ratios, and Prandtl numbers, thereby bringing a step change to RANS capabilities in turbulent conjugate heat transfer analysis.}, number={3}, journal={Journal of Turbulence}, author={Yang, Gaoqiang and Iacovides, Hector and Craft, Timothy and Apsley, David}, year={2021}, month=mar, pages={180–207}, language={en} }


 @inproceedings{Yoder_2016, address={San Diego, California, USA}, title={Comparison of Turbulent Thermal Diffusivity and Scalar Variance Models}, ISBN={978-1-62410-393-3}, url={https://arc.aiaa.org/doi/10.2514/6.2016-1561}, DOI={10.2514/6.2016-1561}, booktitle={54th AIAA Aerospace Sciences Meeting}, publisher={American Institute of Aeronautics and Astronautics}, author={Yoder, Dennis A.}, year={2016}, month=jan, language={en} }


 @article{Lewis_Hickey_2023, title={Conjugate Heat Transfer in High-Speed External Flows: A Review}, volume={37}, ISSN={0887-8722, 1533-6808}, DOI={10.2514/1.T6763}, number={4}, journal={Journal of Thermophysics and Heat Transfer}, author={Lewis, Mikaela T. and Hickey, Jean-Pierre}, year={2023}, month=oct, pages={697–712}, language={en} }


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%END JPH%%%%%%%%%%%%%%%%%%%%%%%%%%%
